Context-Guided Diffusion for Out-of-Distribution Molecular and Protein Design

Generative models have the potential to accelerate key steps in the discovery of novel molecular therapeutics and materials. Diffusion models have recently emerged as a powerful approach, excelling at unconditional sample generation and, with data-driven guidance, conditional generation within their training domain. Reliably sampling from high-value regions beyond the training data, however, remains an open challenge -- with current methods predominantly focusing on modifying the diffusion process itself. In this paper, we develop context-guided diffusion (CGD), a simple plug-and-play method that leverages unlabeled data and smoothness constraints to improve the out-of-distribution generalization of guided diffusion models. We demonstrate that this approach leads to substantial performance gains across various settings, including continuous, discrete, and graph-structured diffusion processes with applications across drug discovery, materials science, and protein design.

==> drafts/_icml2024/3_method_leos_version.tex <==

\section{Context-Guided Diffusion Models}
\label{sec:method}

% \begin{figure*}[t!]
% \centering
%     \begin{minipage}{0.3\textwidth}
%       \subcaptionbox{A}{\includegraphics[height=8cm, width=\linewidth]{example-image-b} }
%     \end{minipage}\hfill
%     \begin{minipage}{0.7\textwidth}
%       \begin{minipage}{\linewidth}
%         \includegraphics[trim={3cm 1cm 3cm 1cm},clip, width=\linewidth]{figures/swiss_roll_ps_reg.pdf}
%         \caption{Parameter-space regularization.}
%       \end{minipage}
    
%       \begin{minipage}{\linewidth}
%         \includegraphics[trim={3cm 1cm 3cm 1cm},clip, width=\linewidth]{figures/swiss_roll_fs_reg.pdf}
%         \caption{Function-space regularization.}
%       \end{minipage} 
%     \end{minipage}

% \caption{One and two images}
% \label{fig:illustration_toy_example}
% \end{figure*}


\begin{figure*}[!t]
  \begin{tabular}{c}
    \subfloat[Training algorithm of the context-aware guidance model.]{
    \begin{minipage}{.32\linewidth}
    \begin{algorithm}[H]
    \setstretch{1.3}
    \caption{One guidance model training epoch with the proposed function-space regularization scheme.}
    \textbf{Given: }{$g_{\theta}, h_\phi,  \sigma_{t},\tau_{t},\Hat{\ybf},\Hat{\xbf},\calL^\ast,\calD,  T$} \;
    
    \For{$(\xbf_0, \ybf)\in\calD$}{        
        $t,\Hat{t}\sim\mathcal{U}(0, T)$\;

        $\xbf_{t}\gets\operatorname{NoisingProcess}(\xbf_0, t)$\;
        
        $\Hat{\xbf}_{t}\gets\operatorname{NoisingProcess}(\Hat{\xbf_0}, \Hat{t})$\;

        $\ybf_\text{pr}\gets  g_{\theta}(\Hat{\xbf}_{t}, \Hat{t})$\;
        
        $ \Hat{\Hbf} \gets  h_\phi(\Hat{\xbf}_{t}, \Hat{t})$\;
        
        $\mathbf{K}_{t} = \sigma_{t} \Hat{\Hbf}_{t}\Hat{\Hbf}_{t}^T+\tau_{t}\mathbf{I}$\;

        $\ell_\text{reg}  \gets -\log \prod_{i=1,2}\calN(\ybf_\text{pr};\mathbf{\Hat{y}}_{i}, \mathbf{K}_{t})$\hspace*{-10pt}\;
        
        $\ell_\text{loss} \gets \calL(\theta, \calD_{t}, \mathcal{T}) + \frac{1}{2 \lambda} ||\theta||_{2}^{2} $\;

        $g_{\theta}\gets\operatorname{Update}(g_{\theta}, \ell_\text{loss} + \ell_\text{reg})$\;
    }
    \end{algorithm}
\end{minipage}%
  }
  \end{tabular}
  \begin{tabular}{c}
    \subfloat[Predictions and samples from an $L2$-regularized guidance model.]{\includegraphics[width=0.65\linewidth]{figures/swiss_roll_ps_reg.png}} \\
    \subfloat[Predictions and samples from a context-aware guidance model.]{\includegraphics[width=0.65\linewidth]{figures/swiss_roll_fs_reg.png}}
  \end{tabular}
  \caption{Panel (a) presents an algorithmic perspective on how the proposed regularization scheme fits into the training loop of a standard guidance model. Panels (b) and (c) illustrate how the regularization scheme affects the functions a guidance model learns. Two regression models with different regularizers are trained on a low-label subset of an illustrative dataset (color-coded crosses). While both fit the training data well, the predictions of the $L_2$-regularized model (b) are overconfident and incorrect in regions beyond the training data. In contrast, a context-aware model (c) is able to leverage unlabeled data sampled uniformly from $[-2.5, 2.5]^2\subset\R^2$ to make more accurate predictions that extrapolate well to near-out-of-distribution regions. The corresponding conditional guided denoising process consistently generates samples that recover a held-out, high-label test set (black crosses). Full experimental details are presented in~\Cref{app:toy_example}.}
  \label{fig:reg_illustration}
\end{figure*}

In the following, we summarize the prevailing approach for training guidance models and highlight its limitations. We then present \emph{context-guided diffusion} (CGD)---a method that leads to more robust conditional gradient estimates that consistently lead to novel samples with improved properties. Specifically, we propose a tractable regularization term that is able to bias guidance model training toward functions that (i) fit the training data well and (ii) revert to domain-appropriate behavior in out-of-distribution settings.
Finally, we highlight that our method is probabilistically motivated and show that it can be recast in a Bayesian framework.

% In this section, we present \emph{context-guided diffusion} (CGD)---a method that produces more robust conditional gradient estimates that consistently lead to novel samples with improved properties.
% We start by summarizing the prevailing approach for training guidance models and highlighting its limitations.
% We then propose a tractable regularization term that is able to bias guidance model training toward functions that (i) fit the training data well and (ii) revert to domain-appropriate behavior in out-of-distribution settings.
% Finally, we highlight that our method is probabilistically motivated and show that it can be recast in a Bayesian framework.

\subsection{Standard Guidance Model Training}
\label{sec:standard_guidance_model_training}

We consider a standard supervised learning setting with timesteps $t=0,...,T$ and $N$ i.i.d. data realizations \mbox{${\calD_{t} = \{(\xbf_{t}^{(n)}, \by^{(n)})\}_{n=1}^{N}}$} of inputs \mbox{$\xbf_{t} \in \calX$} and targets \mbox{$\ybf \in \calY$}.
Furthermore, we define the guidance network \mbox{$f(\cdot \,; \theta) \defines \theta_{L}h(\cdot \,; \theta_{h})$} with $\theta \defines \{ \theta_{h}, \theta_{L} \}$ as the composition of an embedding model \mbox{$h(\cdot \,; \theta_{h}):\calX\to\R^d$} and an affine output head $\theta_L:\R^d\to\calY$.
Finally, we consider a parametric observation model \mbox{$\Bar{p}_{t}(\by \vbar \xbf_{t}; f(\cdot ; \theta))$} defined in terms for the guidance network \mbox{$f(\cdot \,; \theta)$}

Conventional supervised learning techniques for training guidance models define the timestep-dependent negative log-likelihood objective,
\begin{align*}
    \calL(\theta, \calD_{\mathcal{T}}, \mathcal{T})
    \defines
    -\sum_{n=1}^{N} \log{\Bar{p}_{\mathcal{T}}(\by^{(n)} \vbar \xbf^{(n)}_{\mathcal{T}} ; f(\cdot ; \theta))}
    %+ \frac{1}{2\lambda} ||\theta||_{2}^{2},
    % -\sum_{n=1}^{(n)} \log{p_{\Ybf | \Xbf, \Theta}(\by^{(n)} \vbar \xbf^{(n)}_{t} , \theta)}.
\end{align*}
where $\mathcal{T} \sim p_{\mathcal{T}}(t)$ is a random timestep, and optimize the parameters $\theta$ by minimizing the objective function
\begin{align}
\label{eq:standard_loss}
    \Bar{\calL}(\theta, \calD_{\mathcal{T}}, \mathcal{T})
    \defines
    \E_{p_{\mathcal{T}}}\left[ \calL(\theta, \calD_{\mathcal{T}}, \mathcal{T}) \right]
    + 
    \frac{1}{2\lambda} ||\theta||_{2}^{2},
\end{align}
where $\lambda\in\R_{+}$ is a hyperparameter that determines the $L_2$-regularization strength.

However, this objective is only able to consider subsets of the input domain $\calX$ for which labeled data is available. 
When these subsets are biased and small, as is often the case in practice, models trained with standard supervised learning objectives are prone to generating incorrect and highly overconfident predictions when exposed to distribution shifts \cite{ovadia2019can, liu2020simple, van2020uncertainty, koh2021wilds, rudner2022tractable, klarner2023drug}.
This issue is exacerbated by the fact that guidance models are trained on noised data points:
Since neural networks are both highly sensitive to noise perturbations \cite{szegedy2013intriguing,goodfellow2014explaining,ho2022classifier} and able to overfit to fully corrupted inputs \cite{zhang2021understanding}, consistently overconfident gradient signals at larger noise scales can accumulate over hundreds of denoising steps.


\subsection{Context-Aware Guidance Models}
\label{sec:regularization_objective}

To improve the reliability of guidance models, we propose a family of timestep-dependent regularizers $R^\ast_{t}$ that favor parameters $\theta$ that encode desirable behavior \mbox{$f(\Hat{\xbf}_{t} \,; \theta)=\Hat{\ybf}\in\mathcal{Y}^M$} on a problem-specific out-of-distribution context set $\Hat{\xbf} \defines \{ \Hat{\xbf}_{t} \}_{t=0}^{T}$ with \mbox{$\Hat{\xbf}_{t}\in\calX^M$}.
While the optimal behavior on out-of-distribution data points is often application-dependent, we find that encouraging uncertain predictions in areas of the input domain with little or no signal from the supervised learning process performs well across settings.
This \emph{Gaussian process prior} maximizes sensitivity at the expense of specificity and enables the conditional denoising process to focus on near out-of-distribution regions with the highest likelihood of containing molecules with improved properties.
%While the specific choice of $\Hat{\ybf}$ is application-dependent, 
%of predictive models evaluated on out-of-distribution data 
%we can construct a broadly applicable prior that places high probability density on parameter values that induce models with high predictive uncertainty on the context set that increases as a function of the timestep $t$.
% To do so, we build on the result in \citet{rudner2023function}, which showed that MAP estimation with domain-informed priors, which can be expressed as $p(\theta \vbar \Hat{\calD}) = \frac{\Hat{p}(\Hat{\ybf} \vbar \Hat{\xbf}, \theta) \Hat{p}(\theta)}{\Hat{p}(\Hat{\ybf} \vbar \Hat{\xbf})}$ by Bayes theorem, only requires specifying a tractable joint distribution $\Hat{p}(\Hat{\ybf} \vbar \Hat{\xbf}, \theta) \Hat{p}(\theta)$.
%To construct a domain-informed auxiliary likelihood function $\Hat{p}(\Hat{\ybf} \vbar \Hat{\xbf}, \theta)$, we extend the prior presented in \citet{rudner2023function}.
To construct such a regularizer, we extend the method proposed in \citet{rudner2023function} and adapt it to the optimization of time-step dependent discriminative models in guided diffusion settings.

We start by constructing an embedding matrix $\Hat{\Hbf}_{t}\in\R^{M\times d}$ for all molecules in the context set $\Hat{\xbf}_{t}$. Our regularizer is agnostic to how these embeddings are derived, so long as they capture relevant structural properties of the input domain. While using foundation models trained on large corpora of unlabeled molecular graphs or protein sequences \cite{lin2022language} would be a sensible choice, we find that a much simpler approach is already sufficient to produce sizeable performance gains in the settings we consider in~\Cref{sec:experiments}. Specifically, we use a fixed set of randomly initialized parameters $\phi$ to obtain \mbox{$\Hat{\Hbf}_{t} = h(\Hat{\xbf}_{t}, \phi)$} from the guidance model's embedding trunk, motivated by the fact that models with suitable inductive biases, such as permutation- or roto-translational invariance, can already produce informative embeddings in a randomly initialized state~\cite{kipf2016semi}.
While it is possible to use the learned parameters $\theta$ directly, we found that optimizing them with respect to the regularization objective resulted in ``feature collapse'' \cite{van2021feature} and worse downstream performance.

We then leverage the inner product of context points in this embedding space to construct the covariance matrix
\begin{align}
\label{eq:covariance_matrix}
\begin{split}
    \mathbf{K}_{t}(\Hat{\Hbf}_{t}, t) = \sigma_{t} \Hat{\Hbf}_{t}\Hat{\Hbf}_{t}^T+\tau_{t}\mathbf{I}.
\end{split}
\end{align}
Here, the covariance scale $\sigma_{t}$ regularizes the smoothness of the functions learned by our guidance model and determines how strongly its predictions can vary between similar out-of-distribution context points. The diagonal scale $\tau_{t}$, on the other hand, specifies how closely the predictions should match the desired behavior $f(\Hat{\xbf}_{t} \,; \theta)=\Hat{\ybf}$.

% In classification settings, $\Hat{\ybf}_{t}$ is given by a zero-logit vector 
%$\Hat{\ybf}=\mathbf{0}$ 
% that encourages equal class probabilities.
Letting $f$ be a standard multi-output regression model consisting of a learned mean function $[f(\hat{\xbf}_{t} ; \theta)]_{1}$ and, optionally, a learned variance function $[f(\hat{\xbf}_{t} ; \theta)]_{2}$, we define the desired behavior as $\Hat{\ybf}_{1} \defines \frac{1}{N}\sum_{n=1}^{N} y^{(n)}$ and $\Hat{\ybf}_{2} \defines \boldsymbol{\sigma_{0}}^{2}$, with $\boldsymbol{\sigma_{0}}^{2}$ a variance hyperparameter, encouraging the predictions of our model to revert to the training set mean and high uncertainty on out-of-distribution data points.
% \begin{align}
%     M = J^T * J
    
%     Phi =  d f (x; theta_h, thets_L) / d theta_L
%     Phi:= "How much does f change, as we change theta_l by one unit"
        
% \end{align}


Putting everything together, we define our regularizer as
\begin{align}
\label{eq:regularizer}
    %&
    R(\theta, f, \hat{\xbf}_{t}, t)
    %\\
    %&
    =
    \sum_{i=1,2 }\log \calN([f(\hat{\xbf}_{t} ; \theta)]_{i} ; \Hat{\ybf}_{i}, \mathbf{K}_{t}(\Hat{\Hbf}_{t}, t)).
    %+ \frac{1}{2\lambda}\|\theta\|_{2}^{2} ,
\end{align}
%where $[f(\hat{\xbf}_{t} ; \theta)]_{1}$ and $[f(\hat{\xbf}_{t} ; \theta)]_{2}$ denote the mean and the variance output of the guidance model, respectively.
Intuitively, this approach can be viewed as enforcing the specified behavior via a Gaussian process with a product kernel in a domain-informed embedding space.
Combining this approach with the supervised loss from \Cref{eq:standard_loss}, we arrive at the modified training objective
\begin{align*}
%\label{eq:fseb_loss}
\begin{split}
    % &
    % \hspace{-7pt}
    \mathcal{L}^\ast(\theta, \calD, \hat{\xbf})
    % \\
    % &
    % \hspace{-4pt}
    =
    % \hspace*{-2pt}
    \E_{p_{\mathcal{T}}}[ \calL(\theta, \calD_{\mathcal{T}}, \mathcal{T})] + \E_{p_{\mathcal{T}}}[ R_{\mathcal{T}}(\theta, f, \hat{\xbf}_{\mathcal{T}}, \mathcal{T}) ]
    % \hspace*{-2pt}\E_{p_T}\left[\calL(\xbf^{\calD}_0, \by^{\calD}, \theta, t) + \Hat{R}_{t}(\theta, f, \hat{\xbf}_{t}, t)\right] 
    %\\
    %&
    % + \frac{1}{2\lambda}\|\theta\|_{2}^{2} .
    % \nonumber 
\end{split}
\end{align*}
% The full regularizer is given by the negative log-likelihood of a multivariate Gaussian distribution with mean $\ybf$ and covariance $\mathbf{K}_{t}(\Hat{\Hbf}_{t}, t)$
% To relate this log prior to more conventional training techniques, we note that we can view MAP estimation with a data-driven prior as maximum likelihood estimation with a context-informed regularizer
% \begin{align*}
% \begin{split}
%     &
%     R^\ast_{t}(\theta, f, \hat{\xbf}_{t}, t)
%     % \\
%     % &
%     % \defines
%     % \E_{p_{T}}\left[ \log p(\theta \vbar \Hat{\calD}, T) \right]
%     % \\
%     % &
%     =
%     - \log \prod_{i=1,2} \calN([f(\hat{\xbf}_{t}]_{i} ; \theta) ; \Hat{\ybf},\mathbf{K}_{t}(\Hat{\Hbf}_{t}, t))
%     % \\
%     % &
%     % =
%     % \sum_{k = 1}^{K} \frac{\tau_{f}}{2} d^{2}_{M}(f(\hat{\xbf}_{T} ; \theta)_{k},  \mathbf{K}_{t}(\Hat{\Hbf}_{t}, t)
%     % \hspace*{-2pt}-\hspace*{-2pt} 
%     % \frac{\tau_{\theta}}{2} \|\theta\|_{2}^{2} ,
%     % \hspace*{-2pt}-\hspace*{-2pt}
%     % \E_{p_{T}}\left[ \sum_{k = 1}^{K} \frac{\tau_{f}}{2} d^{2}_{M}(f(\hat{\xbf}_{T} ; \theta)_{k}, K(\hat{\xbf}_{T}, \hat{\xbf}_{T} ; \phi_{0})) \right] 
%     % \hspace*{-2pt}-\hspace*{-2pt} 
%     % \frac{\tau_{\theta}}{2} \|\theta\|_{2}^{2} ,
% \end{split}
% \end{align*}
% % \begin{align}
% %     R(\theta, f, \hat{\xbf})
% %     \defines
% %     \hspace*{-2pt}-\hspace*{-2pt}
% %     \frac{\tau_{f}}{2} d^{2}_{M}(f(\hat{\xbf}_{t} ; \theta)_{k}, K(\hat{\xbf}_{t}, \hat{\xbf}_{t} ; \phi)) ,
% % \end{align}

\paragraph{Implementation.}
Since our method is highly modular and does not require any changes to the guidance model itself, it can be easily integrated into standard guidance model training regimes:
At each iteration, we sample a mini-batch from the context set $\Hat{\xbf}_{t}$ and perturb it with the same noising process as the unconditional diffusion model in~\Cref{eq:forward_noising_process}.
We then perform a gradient-free forward pass of the embedding trunk $h(\Hat{\xbf}_{t}, \phi)$ to derive the embeddings $\Hat{\Hbf}$ and construct the covariance matrix $\mathbf{K}_{t}(\Hat{\Hbf}_{t}, t)$. Finally, we evaluate the guidance model $f(\hat{\xbf}_{t} ; \theta)$ on the context batch to compute the regularization term in~\Cref{eq:regularizer}.
An algorithmic overview of this process is provided in~\Cref{fig:reg_illustration}.

Since the risk of miscalibrated gradient estimates is particularly high in the earlier stages of the sample generation process---where highly diffused input points are associated with the labels of the corresponding un-noised points--- we ensure that our regularizer is able to take the noise level $\beta_t$ into account.
Specifically, we increase $\tau_{t}$ with the same schedule as the noise scales $\beta_t$ to penalize overconfident predictions as context points approach the target distribution $\calN(\mathbf{0},\mathbf{I})$.
Similarly, as the distinction between in- and out-of-distribution points becomes less meaningful at larger noise levels, we decrease $\sigma_{t}$ with an inverted schedule.

% As shown in \citet{rudner2023function}, optimizing this objective corresponds to MAP estimation with a data-driven prior as shown in \Cref{eq:map_domain}.
% Finally, using the learned parameters $\theta^\ast$ as shown in \Cref{eq:domain_informed_guidance} allows us to perform domain-informed guided diffusion.

% We modify the reverse-time SDE in~\Cref{eq:guided_denoising_process} to incorporate uncertainty about the label $\ybf$.
% Specifically, we define the SDE as
% \begin{align}
% \label{eq:guided_denoising_process_modified}
% \begin{split}
%     % \mathrm{d} \mathbf{\Bar{X}}_{t}
%     % =&
%     % \beta_{T-t} \left\{\frac{1}{2} \mathbf{\Bar{X}}_{t} +\nabla \mathcal{S}(\Bar{\xbf}_{t}) \right\} \mathrm{d} t
%     % % \\
%     % % &
%     % % \qquad\qquad\quad
%     % + \sqrt{\beta_{T-t}} \mathrm{d} \mathbf{B}_{t} ,
%     \mathrm{d} \mathbf{X}_{t} 
%     = 
%     -\beta_{t} \left\{\frac{1}{2} \mathbf{X}_{t} + \nabla \mathcal{S}(\Xbf_{t}) \right\} \mathrm{d} t + \sqrt{\beta_{t}} \mathrm{d} \mathbf{B}_{t}.
% \end{split}
% \end{align}
% with
% \begin{align}
%     \mathcal{S}(\Xbf_{t})
%     \defines
%     \E_{\pi} \left[ \log p_{t}\left(\Xbf_{t}\vbar \Ybf\right) \right] ,
% \end{align}
% where $p_{t}\left(\xbf_{t}\vbar \ybf\right)$ is as defined above and $\pi(\ybf) \defines p(\ybf \vbar \xbf_{t})$ is a distribution over the model labels $\ybf$.
% % This is particularly important when labeled data is scarce and errors can accumulate over hundreds of denoising steps.
% Standard guidance is recovered for \mbox{$p(\ybf \vbar \xbf_{t}) \defines \delta(\ybf - \ybf^\ast)$} with $\ybf^\ast \defines \arg\max_{\ybf} p(\ybf \vbar \xbf_{t})$.
% Following \Cref{eq:conditional_score}, we obtain
% \begin{align}
% \begin{split}
%     % &
%     \nabla \mathcal{S}(\Xbf_{t})
%     % \\
%     &
%     =
%     \nabla \int p(\ybf \vbar \xbf_{t}) \log p_{t}\left(\xbf_{t} \vbar \ybf \right) \dee \ybf
%     \\
%     &
%     =
%     \nabla \int p(\ybf \vbar \xbf_{t}) \log p_{t}\left(\ybf \vbar \xbf_{t} \right) \dee \ybf
%     % \\
%     % &
%     % \qquad
%     + \nabla \log p_{t}(\xbf_{t}) .
% \end{split}
% \end{align}
% % \begin{align}
% % \begin{split}
% %     % &
% %     \nabla \mathcal{S}(\Xbf_{t})
% %     % \\
% %     &
% %     =
% %     \nabla \int p(\ybf \vbar \xbf_{t}) \log p_{t}\left(\xbf_{t} \vbar \ybf \right) \dee \ybf
% %     \\
% %     &
% %     =
% %     \nabla \int p(\ybf \vbar \xbf_{t}) \log p_{t}\left(\ybf \vbar \xbf_{t} \right) \dee \ybf
% %     % \\
% %     % &
% %     % \qquad
% %     + \nabla \log p_{t}(\xbf_{t}) .
% % \end{split}
% % \end{align}
% Under this formulation, we recover the original reverse-time SDE approximation for \mbox{$q(\theta) \defines \delta(\theta - \Bar{\theta})$}, where $\delta(\cdot)$ is the Dirac delta function and $\Bar{\theta}$ denotes the maximum likelihood estimate of the parameters obtained via training on data $\calD$.
% If, instead, we specify \mbox{$q(\theta) \defines p(\theta \vbar \calD)$}, where $p(\theta \vbar \calD)$ is the posterior distribution over the model parameters given data $\calD$, $\mathcal{S}(\xbf_{t})$ becomes the well-established Bayes risk.
% However, since computing $p(\theta \vbar \calD)$ and the integral under $p(\theta \vbar \calD)$ are not in general tractable, we can instead choose $q(\theta) \defines \delta(\theta - \theta^\ast)$, where $\theta^\ast$ is the maximum a posteriori (\textsc{MAP}) estimate $\theta^\ast \defines \arg\max_{\theta} p(\theta \vbar \calD)$, which yields
% \begin{align}
% \begin{split}
%     % \hspace*{-10pt}
%     % &
%     \nabla \mathcal{S}^\ast(\xbf_{t})
%     % \\
%     &
%     =
%     \nabla \log p_{t}(\ybf \vbar \xbf_{t}, \theta^\ast )
%     % \\
%     % &
%     % \qquad
%     + \nabla \log p_{t}(\xbf_{t}) .
% \end{split}
% \end{align}

% Using this \textsc{MAP} estimate allows us to construct a prior distribution $p(\theta)$ 
% %to influence the learned parameters via
% to encode suitable modeling preferences
% \begin{align}
%     \theta^\ast \defines \arg\max_{\theta} p(\theta \vbar \calD) = \arg\max_{\theta}  p(\calD \vbar \theta) p(\theta).
% \end{align}

% In practice, guided diffusion models require a parametric model of $p_{t}\left(\mathbf{X}_{t}\vbar \ybf\right)$ to use guidance in reverse-time SDEs.
% To reflect this fact and reveal implicit modeling assumptions made when specifying parametric guidance models, we define a {distributional parametric} reverse-time SDE,
% \begin{align}
% % \SwapAboveDisplaySkip
% \label{eq:guided_denoising_process_modified}
% \begin{split}
%     % \mathrm{d} \mathbf{\Bar{X}}_{t}
%     % =&
%     % \beta_{T-t} \left\{\frac{1}{2} \mathbf{\Bar{X}}_{t} +\nabla \mathcal{S}(\Bar{\xbf}_{t}) \right\} \mathrm{d} t
%     % % \\
%     % % &
%     % % \qquad\qquad\quad
%     % + \sqrt{\beta_{T-t}} \mathrm{d} \mathbf{B}_{t} ,
%     \mathrm{d} \mathbf{X}_{t} 
%     = 
%     -\beta_{t} \left\{\frac{1}{2} \mathbf{X}_{t} + \mathcal{S}(\Xbf_{t}) \right\} \mathrm{d} t + \sqrt{\beta_{t}} \mathrm{d} \mathbf{B}_{t} ,
% \end{split}
% \end{align}
% with a tailored score function%\vspace*{-7pt}
% \begin{align}
% % \SwapAboveDisplaySkip
%     \mathcal{S}(\Xbf_{t})
%     &
%     \defines
%     \nabla \log p_{t}(\Xbf_{t} \vbar \bm{v}; f(\cdot ; \theta) )
%     \\
%     &
%     =
%     \nabla \log p_{t}(\bm{v} \vbar \Xbf_{t}; f(\cdot ; \theta) )
%     % \\
%     % &
%     % \qquad
%     + \nabla \log p_{t}(\Xbf_{t}) .
%     \nonumber
% \end{align}\\[-13pt]
% defined in terms of a parametric value distribution
% \begin{align}
%     p_{t}(\bm{v} \vbar \Xbf_{t}; f(\cdot ; \theta) )
%     \defines
%     \calN(\bm{v} ; \mathbb{E}[u(\Xbf_{t} ; f(\cdot ; \theta))], \sigma^{2} I) ,
% \end{align}
% where the expectation is defined with respect to the learned guidance model $p(\ybf \vbar \Xbf_{t}  ; f(\cdot ; \theta))$, so that
% \begin{align}
%     u(\Xbf_{t}; f(\cdot ; \theta))
%     =
%     \int p(\ybf \vbar \Xbf_{t}  ; f(\cdot ; \theta)) \, u(\ybf) \dee \ybf .
% \end{align}
% Letting $u(\ybf) \defines -\exp(-\lambda \ybf) / \lambda$, an exponential utility function with $\lambda<0$,


% We recover the conventional reverse-time SDE approximation for \mbox{$q(\theta) \defines \delta(\theta - \Bar{\theta})$}, where $\delta(\cdot)$ is the Dirac delta function and $\Bar{\theta}$ denotes the maximum likelihood estimate of the parameters obtained via training on the labeled dataset $\calD$.





% % %%%%%%% BACKUP
% In practice, diffusion models require a parametric model of $p_{t}\left(\mathbf{X}_{t}\vbar \ybf\right)$ for conditional sample generation.
% To reflect this fact and emphasize the implicit modeling assumptions made when specifying parametric guidance models, we define a {parametric} reverse-time SDE,
% \begin{align}
% % \SwapAboveDisplaySkip
% \label{eq:guided_denoising_process_modified}
% \begin{split}
%     % \mathrm{d} \mathbf{\Bar{X}}_{t}
%     % =&
%     % \beta_{T-t} \left\{\frac{1}{2} \mathbf{\Bar{X}}_{t} +\nabla \mathcal{S}(\Bar{\xbf}_{t}) \right\} \mathrm{d} t
%     % % \\
%     % % &
%     % % \qquad\qquad\quad
%     % + \sqrt{\beta_{T-t}} \mathrm{d} \mathbf{B}_{t} ,
%     \mathrm{d} \mathbf{X}_{t} 
%     = 
%     -\beta_{t} \left\{\frac{1}{2} \mathbf{X}_{t} + \mathcal{S}(\Xbf_{t}) \right\} \mathrm{d} t + \sqrt{\beta_{t}} \mathrm{d} \mathbf{B}_{t} ,
% \end{split}
% \end{align}
% with an expected score function\vspace*{-7pt}
% \begin{align}
% % \SwapAboveDisplaySkip
%     \mathcal{S}(\Xbf_{t})
%     \defines
%     \int q(\theta) \nabla \log p_{t}(\Xbf_{t} \vbar \ybf; f(\cdot ; \theta) ) \dee \theta ,
% \end{align}\\[-13pt]
% a parametric observation model $p_{t}\left(\Xbf_{t} \vbar \ybf; f(\cdot ; \theta) \right)$ defined in terms of a {\em guidance model} $f(\Xbf_{t} ; \theta)$, and a distribution over the model parameters $q(\theta)$.
% % This is particularly important when labeled data is scarce and errors can accumulate over hundreds of denoising steps.
% % Noting that
% % \begin{align}
% % \begin{split}
% % \label{eq:conditional_score}
% %     &
% %     \log p_{t}\left(\Xbf_{t} \vbar \ybf; f(\cdot ; \theta) \right)
% %     \\
% %     &
% %     =
% %     \log p_{t}(\ybf \vbar \Xbf_{t}; f(\cdot ; \theta)) + \log p_{t}(\Xbf_{t}) + \log p_{t}(\ybf \vbar \theta) ,
% % \end{split}
% % \end{align}
% Following~\Cref{eq:conditional_score}, we obtain a {\em distributional parametric guidance function}
% \begin{align}
% % \SwapAboveDisplaySkip
% \label{eq:distributional_guidance}
% % \begin{split}
%     % &
%     \mathcal{S}(\Xbf_{t})
%     % \\
%     &
%     =
%     \int q(\theta) \nabla \log p_{t}(\Xbf_{t} \vbar \ybf; f(\cdot ; \theta) ) \dee \theta
%     \\
%     &
%     =
%     \int q(\theta) \nabla \log p_{t}(\ybf \vbar \Xbf_{t}; f(\cdot ; \theta) ) \dee \theta
%     % \\
%     % &
%     % \qquad
%     + \nabla \log p_{t}(\Xbf_{t}) . \nonumber
% % \end{split}
% \end{align}
% For a derivation, see \Cref{app:method_derivation}.
% % We refer to this family of guidance functions as {\em distributional parametric guidance}.
% We recover the conventional reverse-time SDE approximation for \mbox{$q(\theta) \defines \delta(\theta - \Bar{\theta})$}, where $\delta(\cdot)$ is the Dirac delta function and $\Bar{\theta}$ denotes the maximum likelihood estimate of the parameters obtained via training on the labeled dataset $\calD$.


% \subsection{A Bayesian Perspective on Distributional Guidance}

% Explicitly including the guidance function parameterization in the SDE allows us to be more transparent about our modeling assumptions and reveals a broader design space for defining parametric guidance models.
% If, for example, we specify \mbox{$q(\theta) \defines p(\theta \vbar \calD)$}, where $p(\theta \vbar \calD)$ is the posterior distribution over the model parameters given labeled data $\calD = \{(\bx_{t}^{(n)},\ybf^{(n)})\}$, $\mathcal{S}(\Xbf_{t})$ becomes the posterior expected score function.
% Choosing the posterior \mbox{$p(\theta \vbar \calD)$} has an intuitive appeal:
% It provides a probabilistically principled approach to incorporating information from labeled data into the guidance model and naturally translates uncertainty about the guidance model parameters into the guidance function.

% Unfortunately, computing $p(\theta \vbar \calD)$ is not in general tractable, but instead of using the full posterior, we can use the {\em most likely parameters under the posterior} as a tractable alternative which---while not reflecting uncertainty about the model parameters---retains the ability to incorporate prior beliefs into the guidance model.
% To use the most likely parameters under the posterior, we let $q(\theta) \defines \delta(\theta - \theta^{\mathrm{MAP}})$, where $\theta^{\mathrm{MAP}}$ is the maximum a posteriori (\textsc{MAP}) estimate,
% \begin{align}
%     \theta^{\mathrm{MAP}} \defines \arg\max_{\theta} p(\theta \vbar \calD) = \arg\max_{\theta}  p(\calD \vbar \theta) p(\theta) ,
% \end{align}
% with prior distribution $p(\theta)$.
% Under the MAP estimate $\theta^\ast$, we obtain the MAP guidance function
% \begin{align*}
% \begin{split}
%     % &
%     \nabla \mathcal{S}^{\mathrm{MAP}}(\Xbf_{t})
%     % \\
%     &
%     =
%     \nabla \log p_{t}(\ybf \vbar \Xbf_{t}, \theta^{\mathrm{MAP}} ; f) + \nabla \log p_{t}(\Xbf_{t}) .
% \end{split}
% \end{align*}
% A commonly used prior is an isotropic Gaussian distribution with \mbox{$p(\theta)=\calN(\theta;\mathbf{0},\lambda\mathbf{I})$}, which favors parameters with small $L_2$-norm.
% While simple and useful, uninformative priors like this only reflect simple inductive biases and are unable to incorporate more sophisticated prior beliefs into model training, making them of limited use for problems in which encoding additional information can be critical.
%for problems where additional information about the modeled domain is available.

%While there is nothing particularly remarkable about this guidance function, its construction provides a blueprint for incorporating relevant task-specific information into the guidance function via informative data-driven priors.
%We will discuss the construction of such priors and the construction of domain-informed guidance functions next.



% \subsection{Domain-Informed Guidance Functions}

% Next, we will build on this formulation to incorporate task-specific information into the guidance function by constructing a {\em domain-informed prior} that places high probability density on parameters that induce predictive models with desirable properties~\citep{rudner2023function}.

% %While it is challenging to construct data-independent informative priors over neural network parameters, we can use domain-specific data to construct informative {\em data-driven priors} that place high probability density on parameters that induce predictive models with desirable properties~\citep{rudner2023function}.

% Given labeled data $\calD$, domain-specific context data $\Hat{\calD}$, and a domain-informed data-driven prior $p(\theta \vbar \Hat{\calD})$, the posterior $p(\theta \vbar \calD, \Hat{\calD})$ reflects both the prior beliefs encoded in $p(\theta \vbar \Hat{\calD})$ as well as the information from the labeled data $\calD$.
% However, since computing $p(\theta \vbar \calD, \Hat{\calD})$ is intractable, we may instead, again, resort to using the MAP estimate,
% \begin{align}
% \label{eq:map_domain}
%     \hspace*{-5pt}\theta^\ast \defines \arg\max_{\theta} p(\theta \vbar \calD, \Hat{\calD}) = \arg\max_{\theta}  p(\calD \vbar \theta) p(\theta \vbar \Hat{\calD}) ,
% \end{align}
% which yields a tractable {\em context-aware guidance function}
% \begin{align*}
% \begin{split}
% \label{eq:domain_informed_guidance}
%     % &
%     \mathcal{S}^{\ast}(\Xbf_{t})
%     % \\
%     &
%     =
%     \nabla \log p_{t}\left(\ybf \vbar \Xbf_{t}, \theta^{\ast} \right) + \nabla \log p_{t}(\Xbf_{t}) ,
% \end{split}
% \end{align*}
% which only differs from previous guidance function in the parameters $\theta^\ast$ in $q(\theta) \defines \delta(\theta - \theta^\ast)$.

% \subsection{Context-Aware Guidance Functions}

% Explicitly including the guidance function parameterization in the SDE allows us to be more transparent about our modeling assumptions and reveals a broader design space for defining parametric guidance models.
% If, for example, we want to incorporate task-specific information into the guidance function, we can specify \mbox{$q(\theta) \defines p(\theta \vbar \calD, \Hat{\calD})$}, where $p(\theta \vbar \calD)$ is the posterior distribution over the model parameters given labeled data $\calD = \{(\bx_{t}^{(n)},\ybf^{(n)})\}$ and $p(\theta \vbar \Hat{\calD})$ is a domain-informed prior.
% Choosing the posterior \mbox{$p(\theta \vbar \calD)$} has an intuitive appeal:
% It provides a probabilistically principled approach to incorporating information from labeled data into the guidance model and, via the domain-informed prior, allows encoding domain knowledge that can be leveraged when only little labeled data is available.

% Unfortunately, computing $p(\theta \vbar \calD, \Hat{\calD})$ is not in general tractable, but instead of using the full posterior, we can use the {\em most likely parameters under the posterior} as a tractable alternative which---while not reflecting uncertainty about the model parameters---retains the ability to incorporate prior beliefs into the guidance model.
% To use the most likely parameters under the posterior $p(\theta \vbar \calD, \Hat{\calD})$, we let $q(\theta) \defines \delta(\theta - \theta^\ast)$, where $\theta^\ast$ is the maximum a posteriori (\textsc{MAP}) estimate,
% \begin{align}
% &\label{eq:map_domain}
%     \hspace*{-5pt}\theta^\ast \defines \arg\max_{\theta} p(\theta \vbar \calD, \Hat{\calD}) = \arg\max_{\theta}  p(\calD \vbar \theta) p(\theta \vbar \Hat{\calD}) ,
% \end{align}
% which yields a tractable {\em domain-informed guidance function}
% \begin{align}
% \begin{split}
% \label{eq:domain_informed_guidance}
%     % &
%     \mathcal{S}^{\ast}(\Xbf_{t})
%     % \\
%     &
%     =
%     \nabla \log p_{t}\left(\ybf \vbar \Xbf_{t}, \theta^{\ast} \right) + \nabla \log p_{t}(\Xbf_{t}) .
% \end{split}
% \end{align}


%While the construction of domain-informed guidance functions appears simple, the challenge in constructing them lies in defining a suitable data-driven prior used for MAP estimation (\Cref{eq:map_domain}).
%Next, we will show how to construct data-driven priors specifically designed for guided diffusion models and present a simple optimization objective for finding $\theta^\ast$.

%The challenge of constructing domain-informed guidance functions lies in defining a suitable data-driven prior used for MAP estimation (\Cref{eq:map_domain}).

% One such scenario is the optimization of parametric guidance models, where we often (i) have access to vast amounts of unlabeled data that span parts of the input space outside of the training domain and (ii) can specify desired properties of guidance functions on out-of-domain data points.
% % In the following, we build on prior work from \citet{rudner2023function} to construct a time-dependent probabilistic model that is able to integrate this additional information into the guidance model training process.
% % Specifically, we construct a regularization term that biases the model towards functions that fit the labeled data well and encode 
% In the next section, we will show how to construct and use data-driven domain-informed prior distributions when training guidance models.

\subsection{Probabilistic Interpretation}
\label{sec:bayesian_interpretation}

\lipsum[1-3]

% where \mbox{$d^{2}_{M}(v, K) \defines v^\top K^{-1} v$} is the squared Mahalanobis distance between $v$ and $\mathbf{0}$.


%\textcolor{red}{Why these are simple to compute and scalable.Why is this ``domain informed''. Why encourage uncertainty? Cite QSAVI.}



%This approach allows us to encode domain-informed prior knowledge through both the form of the  functional prior and the set of context points that we enforce it on. 

% \subsection{Domain-Informed Guidance Models as Bayesian Inference}


%\textcolor{red!50!black}{TO DO}


% ------------ PRIOR TEXT ------------

% Consider the standard supervised learning setting with $N$ i.i.d. data realizations \mbox{${\calD = \{\xbf^{(n)}_0, \by^{(n)}\}_{n=1}^{(n)}} = (\xbf^\calD_0, \mathbf{y}^\calD)$} of inputs \mbox{$\xbf_{t} \in \calX$} and targets \mbox{$\Ybf \in \calY$} with input space \mbox{$\calX \subseteq \real^D$} and target space \mbox{$\calY \subseteq \real^K$} for regression and \mbox{$\calY \subseteq \{0, 1\}^K$} for classification tasks with $K$ classes.
% Further, define a parametric observation model $p_{\Ybf | \Xbf, \Theta}(\by \vbar \xbf, \theta; f)$ with mapping \mbox{$f(\cdot \,; \theta) \defines h(\cdot \,; \theta_{h}) \theta_{L}$}.

% Conventional supervised learning training routines involve minimization of the negative log-likelihood objective function
% \begin{align*}
% % \label{eq:map}
%     \calL(\theta, \xbf_{\calD}, \by_{\calD})
%     =
%     -\sum_{n=1}^{(n)} \log{p_{\Ybf | \Xbf, \Theta}(\by^{(n)}_{\calD} \vbar \xbf^{(n)}_{\calD} , \theta)}
% \end{align*}
% with respect to $\theta$.

% To learn models that exhibit improved generalization under covariate shifts and have well-calibrated predictive uncertainty estimates, we consider training with a domain-informed regularizer $R(\theta, f, \hat{\xbf})$ that favors solutions that induce predictive functions with high predictive uncertainty on a domain-specific set of input points $\hat{\xbf}$.
% The resulting optimization objective is given by
% \begin{align*}
%     &
%     \calF(\theta, \xbf_{\calD}, \by_{\calD})
%     \\
%     % ~
%     &
%     =
%     \E_{q_{\varepsilon}}\bigg[
%     -\sum_{n=1}^{(n)} \log{p_{\Ybf | \Xbf, \Theta}(\by^{(n)}_{\calD} \vbar \xbf^{(n)}_{\calD} , \theta + \varepsilon)} + R(\theta, f, \hat{\xbf}) \bigg] ,
% \end{align*}
% where $\varepsilon \sim \calN(\varepsilon ; 0, \gamma)$ for some fixed, small $\gamma$ (e.g., $\gamma = 10^{-10}$).

% The specific functional form of the regularizer depends on the prediction problem.
% For classification tasks, we consider the negative squared Mahalanobis distance penalty proposed in \citet{rudner2023function}:
% \begin{align}
%     R(\theta, f, \hat{\xbf})
%     \defines
%     \hspace*{-2pt}-\hspace*{-2pt}
%     \sum_{k = 1}^{K} \frac{\tau_{f}}{2} d^{2}_{M}(f(\hat{\xbf} ; \theta)_{k}, K(\hat{\xbf}, \hat{\xbf} ; \phi_{0})) 
%     \hspace*{-2pt}-\hspace*{-2pt} 
%     \frac{\tau_{\theta}}{2} \|\theta\|_{2}^{2} ,
% \end{align}
% where \mbox{$d^{2}_{M}(v, K) \defines v^\top K^{-1} v$} is the squared Mahalanobis distance between $v$ and $\mathbf{0}$.
% For regression tasks, we consider
% % \begin{align}
% %     XXX .
% % \end{align}

%\subsection{Domain-Aware Guidance as Posterior Predictive Gradient Marginalization}

% \TR{
% \begin{itemize}
%     \item
%     Show that we can view gradient in guidance as gradient of the likelihood under the mode the parameter posterior (conditioned on training data and context data)
%     \item
%     Show that guidance update follows exactly from Gaussian marginalization
% \end{itemize}
% }

% To provide an intuition for domain-informed guidance, we show that we can frame the sampling process as marginalization over the gradients of a Bayesian posterior predictive distribution.
% To do so, first, we note that the training neural networks using the regularized objective in \Cref{xxx} corresponds to approximating a posterior distribution over neural network parameters, $p(\theta \vbar \calD, \hat{\calD})$, where \mbox{${\hat{\calD} = \{\hat{\xbf}^{(m)}, \hat{\by}^{(m)}\}_{m=1}^M} = (\hat{\xbf}, \hat{\by})$}.

% Next, we note that guided diffusion can be viewed as marginalization over gradients of a specific loss function:
% \begin{align}
% \begin{split}
%     % &
%     p(\xbf_{t-1} \vbar \xbf_{t})
%     % \\
%     &
%     =
%     \int p(\xbf_{t-1} \vbar \xbf_{t}, \mathbf{z}_{t}) p(\mathbf{z}_{t}) \,\dee \mathbf{z}_{t}
%     \\
%     &
%     =
%     \int \calN(\xbf_{t-1} ; \bmu_{t}(\xbf_{t}) + \bSigma_{t} \mathbf{z}_{t} , \sqrt{\alpha} \bSigma_{t})
%     \\
%     &
%     \qquad~~
%     \cdot \calN(\mathbf{z}_{t} ; \mathbf{g}_{t}(\xbf_{t},\ybf), \gamma \Sigma^{-1} ) \,\dee \mathbf{z}_{t}
%     \\
%     &
%     =
%     \calN(\xbf_{t-1} ; \bmu_{t} + \bSigma_{t}\mathbf{g}_{t}(\xbf_{t},\ybf), \bSigma_{t}) ,
% \end{split}
% \end{align}
% where $\gamma = \frac{1 - \sqrt{\alpha}}{\alpha}$ for $0 < \alpha < 1$, and $\mathbf{g}_{t}(\xbf_{t},\ybf)$ is as defined before.
% This is the standard guided diffusion distribution, but this derivation does not require any first-order approximations.
% Finally, instead of using the gradient of a conventionally trained---deterministic---guidance model, we consider the gradient with respect to $\xbf$ under the {\em expected} negative log-likelihood, where the expectation is computed under a Bayesian posterior distribution over the neural network parameters, that is,
% \begin{align}
%     \mathbf{g}^{\mathrm{Bayes}}(\xbf_{t},\ybf)
%     =
%     \nabla_{\xbf} \E_{p_{\Theta | \calD, \hat{\calD}}}[\calL(\Theta, \xbf, \by)]|_{\xbf=\xbf_{t}} .
% \end{align}
% Since computing $p(\theta \vbar \calD, \hat{\calD})$ is not in general tractable, we need to approximate the posterior.
% By minimizing $\calF(\theta, \xbf_{\calD}, \by_{\calD})$ in \Cref{xxx} with respect to $\theta$, we obtain such an approximation.

% Domain-aware guidance using these parameters is then given by
% \begin{align}
%     \calN(\xbf_{t-1} ; \bmu_{t} + \bSigma_{t}\hat{\mathbf{g}}^{q}_{t}(\xbf_{t},\ybf), \bSigma_{t})
% \end{align}
% with the unbiased Monte Carlo gradient estimate
% \begin{align}
%     \hat{\mathbf{g}}^{q}(\xbf_{t},\ybf)
%     =
%     \frac{1}{S} \sum_{s = 1}^{s} \nabla_{\xbf} \calL(\theta + \varepsilon^{(s)}, \xbf, \by) ]|_{\xbf = \xbf_{t}} ,
% \end{align}
% where $\varepsilon^{(s)} \sim \calN(\varepsilon ; 0, \gamma)$




% By favoring posterior distributions $p_{\Theta\vert\calD}$ that are able to reconcile the signal from a small, labeled dataset with pre-specified modeling preferences, our method biases the training of this guidance model towards functions that are likely to perform well across larger subsets of the input domain.

% Since computing $p(\theta \vbar \calD, \hat{\calD})$ is not in general tractable, we need to approximate the posterior.
% By minimizing $\calF(\theta, \xbf_{\calD}, \by_{\calD})$ in \Cref{xxx} with respect to $\theta$, we obtain such an approximation.

% Domain-aware guidance using these parameters is then given by
% \begin{align}
%     \calN(\xbf_{t-1} ; \bmu_{t} + \bSigma_{t}\hat{\mathbf{g}}^{q}_{t}(\xbf_{t},\ybf), 2 \bSigma_{t})
% \end{align}
% with the unbiased Monte Carlo gradient estimate
% \begin{align}
%     \hat{\mathbf{g}}^{q}(\xbf_{t},\ybf)
%     =
%     \frac{1}{S} \sum_{s = 1}^{s} \nabla_{\xbf} \calL(\theta + \varepsilon^{(s)}, \xbf, \by) ]|_{\xbf = \xbf_{t}} ,
% \end{align}
% where $\varepsilon^{(s)} \sim \calN(\varepsilon ; 0, \gamma)$


% To do so, first, we note that the training neural networks using the regularized objective in \Cref{xxx} corresponds to approximating a posterior distribution over neural network parameters, $p(\theta \vbar \calD, \hat{\calD})$, where \mbox{${\hat{\calD} = \{\hat{\xbf}^{(m)}, \hat{\by}^{(m)}\}_{m=1}^M} = (\hat{\xbf}, \hat{\by})$}.

% When using guidance in diffusion models, the goal is to generate samples that are representative of the training distribution and yet novel.
% Standard guidance functions used in the literature, do not necessarily have the ability to enable generation of such samples.
% This is because, in order to generate samples that reflect properties of the training distribution, but are also meaningfully different, guidance functions need to be able to generalize under covariate shifts.
% That is, in order for guidance functions to encourage the generation of samples that are meaningfully different from samples in the training distribution, the guidance function needs to place high probability density on samples that are related to the training data while also being meaningfully different.
% Neural networks trained with standard supervised learning routines have been shown to generalize poorly under covariate shifts, meaning that they do not provide a good model for recognizing related but meaningfully distinct points in input space.
% This shortcoming creates a problem for classifier guidance in diffusion models.
% In order for guidance functions in diffusion models to meaningfully improve generation, they need to be able to extract a meaningful signal from noisy input points and generalize distribution shifts.

% We propose a simple regularizer that can be used to train classifiers that lead to significantly improved guidance functions.
% We then show that this simple addition to standard supervised learning routines can be viewed as performing approximate Bayesian inference with a domain-informed data-driven prior over the neural network parameters.

% \TR{
% \begin{itemize}
%     \item
%     Outline what kinds of properties we need in guidance functions
%     \item
%     Show how to train a model that has the desired properties
%     \begin{itemize}
%         \item
%         Show that training just requires additional regularizer (show for regression and classification, which require different priors)
%         \item 
%         Show how to use a plug-and-play regularizer
%     \end{itemize}
% \end{itemize}
% }





==> drafts/_icml2024/3_method_old.tex <==
\section{Domain-Informed Guided Diffusion}
\label{sec:method}

% \begin{figure*}[t!]
% \centering
%     \begin{minipage}{0.3\textwidth}
%       \subcaptionbox{A}{\includegraphics[height=8cm, width=\linewidth]{example-image-b} }
%     \end{minipage}\hfill
%     \begin{minipage}{0.7\textwidth}
%       \begin{minipage}{\linewidth}
%         \includegraphics[trim={3cm 1cm 3cm 1cm},clip, width=\linewidth]{figures/swiss_roll_ps_reg.pdf}
%         \caption{Parameter-space regularization.}
%       \end{minipage}
    
%       \begin{minipage}{\linewidth}
%         \includegraphics[trim={3cm 1cm 3cm 1cm},clip, width=\linewidth]{figures/swiss_roll_fs_reg.pdf}
%         \caption{Function-space regularization.}
%       \end{minipage} 
%     \end{minipage}

% \caption{One and two images}
% \label{fig:illustration_toy_example}
% \end{figure*}


\begin{figure*}[!t]
  \begin{tabular}{c}
    \subfloat[Training algorithm of the domain-informed guidance model.]{
    \begin{minipage}{.32\linewidth}
    \begin{algorithm}[H]
    \setstretch{1.3}
    \caption{One guidance model training epoch with the proposed function-space regularization scheme.}
    \textbf{Given: }{$g_{\theta}, h_\phi,  \sigma_{t},\tau_{t},\Hat{\ybf},\Hat{\xbf},\calL^\ast,\calD,  T$} \;
    
    \For{$(\xbf_0, \ybf)\in\calD$}{        
        $t,\Hat{t}\sim\mathcal{U}(0, T)$\;

        $\xbf_{t}\gets\operatorname{NoisingProcess}(\xbf_0, t)$\;
        
        $\Hat{\xbf}_{t}\gets\operatorname{NoisingProcess}(\Hat{\xbf_0}, \Hat{t})$\;

        $\ybf_\text{pr}\gets  g_{\theta}(\Hat{\xbf}_{t}, \Hat{t})$\;
        
        $ \Hat{\Hbf} \gets  h_\phi(\Hat{\xbf}_{t}, \Hat{t})$\;
        
        $\mathbf{K}_{t} = \sigma_{t} \Hat{\Hbf}_{t}\Hat{\Hbf}_{t}^T+\tau_{t}\mathbf{I}$\;

        $\ell_\text{reg}  \gets -\log \prod_{i=1,2}\calN(\ybf_\text{pr};\mathbf{\Hat{y}}_{i}, \mathbf{K}_{t})$\hspace*{-10pt}\;
        
        $\ell_\text{loss} \gets \calL(\theta, \calD_{t}, \mathcal{T}) + \frac{1}{2 \lambda} ||\theta||_{2}^{2} $\;

        $g_{\theta}\gets\operatorname{Update}(g_{\theta}, \ell_\text{loss} + \ell_\text{reg})$\;
    }
    \end{algorithm}
\end{minipage}%
  }
  \end{tabular}
  \begin{tabular}{c}
    \subfloat[Predictions and samples from a parameter-space regularized guidance model.]{\includegraphics[width=0.65\linewidth]{figures/swiss_roll_ps_reg.png}} \\
    \subfloat[Predictions and samples from a function-space regularized guidance model.]{\includegraphics[width=0.65\linewidth]{figures/swiss_roll_fs_reg.png}}
  \end{tabular}
  \caption{Panel (a) presents an algorithmic perspective on how the proposed regularization scheme fits into the training loop of a standard guidance model. Panel (b) and (c) illustrate how the regularization scheme affects the functions a guidance model learns. Two regression models with different regularizers are trained on a low-label subset of the Swiss roll dataset (color-coded crosses). While both fit the data well, the predictions of the parameter space-regularized model (b) are overconfident and incorrect in regions beyond the training data. In contrast, the function-space-regularized model (c) yields predictions that are better calibrated and cover the held-out high-label subset (black crosses). The corresponding guided denoising process consistently generates samples from this region. Full experimental details are presented in~\Cref{app:toy_example}.}
  \label{fig:reg_illustration}
\end{figure*}

In this section, we present \emph{domain-informed guidance}---a method that yields more robust conditional denoising processes that consistently generate novel samples with desirable properties.
%extrapolative generation.
% To build an intuition for this approach, we first show that the conditional sampling process in \Cref{eq:conditiona_transition_kernel} can be reframed as marginalization over a latent random variable $\zbf_{t}$ distributed according to a conditional prior, $p_{t}(\zbf_{t} \vbar \ybf)$. %, conditioned on labels $\ybf$.
First, we will introduce a distributional parametric reverse-time SDE formulation.
Next, we will present a Bayesian perspective on distributional guidance and use it to motivate domain-informed guidance functions.
Finally, we will show how to encode domain information into guided diffusion models by training guidance models with a domain-informed prior.


% \subsection{Guidance as Marginalization}
% \label{sec:guidance_marginalization}

% To derive guided diffusion from marginalization alone, we introduce an alternative transition kernel conditioned on a realization of a random variable $\mathbf{Z}_{t}$,
% \begin{align}
%      p_{t}(\xbf_{t-1} \vbar \xbf_{t}, \mathbf{z}_{t})
%      \defines
%      \calN(\xbf_{t-1} ; \bmu_{t}(\xbf_{t}) + \bSigma_{t} \mathbf{z}_{t} , {\alpha_{t}} \bSigma_{t}) ,
% \end{align}
% with \mbox{$0 < \alpha_{t} < 1$}.
% Using an uninformative prior
% % \mbox{$
% \begin{align}
%     p_{t}(\mathbf{z}_{t})
%     \defines
%     \calN(\mathbf{z}_{t} ; \mathbf{0}, (1 - \alpha_{t}) \bSigma^{-1}_{t} ) ,
% \end{align}
% % $}
% marginalization over $\mathbf{Z}_{t}$ with
% \begin{align}
% \begin{split}
%     % &
%     p_{t}(\xbf_{t-1} \vbar \xbf_{t}, \ybf)
%     % \\
%     % &
%     = \int  p_{t}(\xbf_{t-1} \vbar \xbf_{t}, \mathbf{z}_{t}) p_{t}(\mathbf{z}_{t}) \,\dee \mathbf{z}_{t}
% \end{split}
% \end{align}
% recovers unguided diffusion with the standard unconditional transition kernel
% % \mbox{$
% \begin{align}
%     p_{t}(\xbf_{t-1} \vbar \xbf_{t}) = \calN(\xbf_{t-1} ; \bmu_{t}(\xbf_{t}), \bSigma_{t}) .
% \end{align}
% % $}
% When using an informative prior defined as
% %\mbox{$
% \begin{align}
%     p_{t}(\zbf_{t} \vbar \ybf)
%     \defines
%     \calN(\mathbf{z}_{t} ; \mathbf{g}_{t}(\xbf_{t}, \ybf), (1 - \alpha_{t}) \bSigma^{-1}_{t}),
% \end{align}
% % $}
% we recover guided diffusion with the standard conditional transition kernel
% % I keep changing this for space reasons
% \begin{align}
% \label{eq:marginalization}
% \begin{split}
%     % &
%     p_{t}(\xbf_{t-1} \vbar \xbf_{t}, \ybf)
%     % \\
%     &
%     = \int  p_{t}(\xbf_{t-1} \vbar \xbf_{t}, \mathbf{z}_{t}) p_{t}(\mathbf{z}_{t} \vbar \ybf) \,\dee \mathbf{z}_{t}
%     % \\
%     % &
%     % =
%     % \int p_{t}(\xbf_{t-1} \vbar \xbf_{t}, \mathbf{z}_{t})\calN(\mathbf{z}_{t} ; \mathbf{g}_{t}(\xbf_{t},\ybf), \gamma_{t} \bSigma^{-1}_{t})\dee \mathbf{z}_{t}
%     \\
%     &
%     =
%     \calN(\xbf_{t-1} ; \bmu_{t} + \bSigma_{t}\mathbf{g}_{t}(\xbf_{t},\ybf), \bSigma_{t}) 
% \end{split}
% \end{align}
% without the need for a first-order approximation.
% %Unlike the standard justification for guided diffusion~\citep{sohl2015deep,dhariwal2021diffusion}, this formulation is exact and does not require the use of a---possibly imprecise---first-order approximation.
% This provides a simple and intuitive interpretation:
% Guided diffusion is obtained by marginalizing over all possible values of $\mathbf{Z}_{t}$ under a time-dependent Gaussian distribution centered around the gradients \mbox{$\mathbf{g}_{t}(\xbf_{t},\ybf)=\nabla \log p_{t}(\ybf \vbar \xbf_{t}, \theta)$}.

\subsection{Distributional Parametric Guided Diffusion}

% We modify the reverse-time SDE in~\Cref{eq:guided_denoising_process} to incorporate uncertainty about the label $\ybf$.
% Specifically, we define the SDE as
% \begin{align}
% \label{eq:guided_denoising_process_modified}
% \begin{split}
%     % \mathrm{d} \mathbf{\Bar{X}}_{t}
%     % =&
%     % \beta_{T-t} \left\{\frac{1}{2} \mathbf{\Bar{X}}_{t} +\nabla \mathcal{S}(\Bar{\xbf}_{t}) \right\} \mathrm{d} t
%     % % \\
%     % % &
%     % % \qquad\qquad\quad
%     % + \sqrt{\beta_{T-t}} \mathrm{d} \mathbf{B}_{t} ,
%     \mathrm{d} \mathbf{X}_{t} 
%     = 
%     -\beta_{t} \left\{\frac{1}{2} \mathbf{X}_{t} + \nabla \mathcal{S}(\Xbf_{t}) \right\} \mathrm{d} t + \sqrt{\beta_{t}} \mathrm{d} \mathbf{B}_{t}.
% \end{split}
% \end{align}
% with
% \begin{align}
%     \mathcal{S}(\Xbf_{t})
%     \defines
%     \E_{\pi} \left[ \log p_{t}\left(\Xbf_{t}\vbar \Ybf\right) \right] ,
% \end{align}
% where $p_{t}\left(\xbf_{t}\vbar \ybf\right)$ is as defined above and $\pi(\ybf) \defines p(\ybf \vbar \xbf_{t})$ is a distribution over the model labels $\ybf$.
% % This is particularly important when labeled data is scarce and errors can accumulate over hundreds of denoising steps.
% Standard guidance is recovered for \mbox{$p(\ybf \vbar \xbf_{t}) \defines \delta(\ybf - \ybf^\ast)$} with $\ybf^\ast \defines \arg\max_{\ybf} p(\ybf \vbar \xbf_{t})$.
% Following \Cref{eq:conditional_score}, we obtain
% \begin{align}
% \begin{split}
%     % &
%     \nabla \mathcal{S}(\Xbf_{t})
%     % \\
%     &
%     =
%     \nabla \int p(\ybf \vbar \xbf_{t}) \log p_{t}\left(\xbf_{t} \vbar \ybf \right) \dee \ybf
%     \\
%     &
%     =
%     \nabla \int p(\ybf \vbar \xbf_{t}) \log p_{t}\left(\ybf \vbar \xbf_{t} \right) \dee \ybf
%     % \\
%     % &
%     % \qquad
%     + \nabla \log p_{t}(\xbf_{t}) .
% \end{split}
% \end{align}
% Under this formulation, we recover the original reverse-time SDE approximation for \mbox{$q(\theta) \defines \delta(\theta - \Bar{\theta})$}, where $\delta(\cdot)$ is the Dirac delta function and $\Bar{\theta}$ denotes the maximum likelihood estimate of the parameters obtained via training on data $\calD$.
% If, instead, we specify \mbox{$q(\theta) \defines p(\theta \vbar \calD)$}, where $p(\theta \vbar \calD)$ is the posterior distribution over the model parameters given data $\calD$, $\mathcal{S}(\xbf_{t})$ becomes the well-established Bayes risk.
% However, since computing $p(\theta \vbar \calD)$ and the integral under $p(\theta \vbar \calD)$ are not in general tractable, we can instead choose $q(\theta) \defines \delta(\theta - \theta^\ast)$, where $\theta^\ast$ is the maximum a posteriori (\textsc{MAP}) estimate $\theta^\ast \defines \arg\max_{\theta} p(\theta \vbar \calD)$, which yields
% \begin{align}
% \begin{split}
%     % \hspace*{-10pt}
%     % &
%     \nabla \mathcal{S}^\ast(\xbf_{t})
%     % \\
%     &
%     =
%     \nabla \log p_{t}(\ybf \vbar \xbf_{t}, \theta^\ast )
%     % \\
%     % &
%     % \qquad
%     + \nabla \log p_{t}(\xbf_{t}) .
% \end{split}
% \end{align}

% Using this \textsc{MAP} estimate allows us to construct a prior distribution $p(\theta)$ 
% %to influence the learned parameters via
% to encode suitable modeling preferences
% \begin{align}
%     \theta^\ast \defines \arg\max_{\theta} p(\theta \vbar \calD) = \arg\max_{\theta}  p(\calD \vbar \theta) p(\theta).
% \end{align}





%%%%%%% BACKUP
In practice, guided diffusion models require a parametric model of $p_{t}\left(\mathbf{X}_{t}\vbar \ybf\right)$ to use guidance in reverse-time SDEs.
To reflect this fact and reveal implicit modeling assumptions made when specifying parametric guidance models, we define a {distributional parametric} reverse-time SDE,
\begin{align}
% \SwapAboveDisplaySkip
\label{eq:guided_denoising_process_modified}
\begin{split}
    % \mathrm{d} \mathbf{\Bar{X}}_{t}
    % =&
    % \beta_{T-t} \left\{\frac{1}{2} \mathbf{\Bar{X}}_{t} +\nabla \mathcal{S}(\Bar{\xbf}_{t}) \right\} \mathrm{d} t
    % % \\
    % % &
    % % \qquad\qquad\quad
    % + \sqrt{\beta_{T-t}} \mathrm{d} \mathbf{B}_{t} ,
    \mathrm{d} \mathbf{X}_{t} 
    = 
    -\beta_{t} \left\{\frac{1}{2} \mathbf{X}_{t} + \mathcal{S}(\Xbf_{t}) \right\} \mathrm{d} t + \sqrt{\beta_{t}} \mathrm{d} \mathbf{B}_{t} ,
\end{split}
\end{align}
with an expected score function\vspace*{-7pt}
\begin{align}
% \SwapAboveDisplaySkip
    \mathcal{S}(\Xbf_{t})
    \defines
    \int q(\theta) \nabla \log p_{t}(\Xbf_{t} \vbar \ybf, \theta ; f ) \dee \theta ,
\end{align}\\[-13pt]
a parametric observation model $p_{t}\left(\Xbf_{t} \vbar \ybf, \theta ; f \right)$ defined in terms of a {\em guidance model} $f(\Xbf_{t} ; \theta)$, and a distribution over the model parameters $q(\theta)$.
% This is particularly important when labeled data is scarce and errors can accumulate over hundreds of denoising steps.
% Noting that
% \begin{align}
% \begin{split}
% \label{eq:conditional_score}
%     &
%     \log p_{t}\left(\Xbf_{t} \vbar \ybf, \theta ; f \right)
%     \\
%     &
%     =
%     \log p_{t}(\ybf \vbar \Xbf_{t}, \theta ; f) + \log p_{t}(\Xbf_{t}) + \log p_{t}(\ybf \vbar \theta) ,
% \end{split}
% \end{align}
This way, we obtain a {\em distributional parametric guidance function}
\begin{align}
% \SwapAboveDisplaySkip
\label{eq:distributional_guidance}
% \begin{split}
    % &
    \mathcal{S}(\Xbf_{t})
    % \\
    &
    =
    \int q(\theta) \nabla \log p_{t}(\Xbf_{t} \vbar \ybf, \theta ; f ) \dee \theta
    \\
    &
    =
    \int q(\theta) \nabla \log p_{t}(\ybf \vbar \Xbf_{t}, \theta ; f ) \dee \theta
    % \\
    % &
    % \qquad
    + \nabla \log p_{t}(\Xbf_{t}) . \nonumber
% \end{split}
\end{align}
For a derivation, see \Cref{app:method_derivation}.
% We refer to this family of guidance functions as {\em distributional parametric guidance}.
We recover the conventional reverse-time SDE approximation for \mbox{$q(\theta) \defines \delta(\theta - \Bar{\theta})$}, where $\delta(\cdot)$ is the Dirac delta function and $\Bar{\theta}$ denotes the maximum likelihood estimate of the parameters obtained via training on the labeled dataset $\calD$.

% \subsection{A Bayesian Perspective on Distributional Guidance}

% Explicitly including the guidance function parameterization in the SDE allows us to be more transparent about our modeling assumptions and reveals a broader design space for defining parametric guidance models.
% If, for example, we specify \mbox{$q(\theta) \defines p(\theta \vbar \calD)$}, where $p(\theta \vbar \calD)$ is the posterior distribution over the model parameters given labeled data $\calD = \{(\bx_{t}^{(n)},\ybf^{(n)})\}$, $\mathcal{S}(\Xbf_{t})$ becomes the posterior expected score function.
% Choosing the posterior \mbox{$p(\theta \vbar \calD)$} has an intuitive appeal:
% It provides a probabilistically principled approach to incorporating information from labeled data into the guidance model and naturally translates uncertainty about the guidance model parameters into the guidance function.

% Unfortunately, computing $p(\theta \vbar \calD)$ is not in general tractable, but instead of using the full posterior, we can use the {\em most likely parameters under the posterior} as a tractable alternative which---while not reflecting uncertainty about the model parameters---retains the ability to incorporate prior beliefs into the guidance model.
% To use the most likely parameters under the posterior, we let $q(\theta) \defines \delta(\theta - \theta^{\mathrm{MAP}})$, where $\theta^{\mathrm{MAP}}$ is the maximum a posteriori (\textsc{MAP}) estimate,
% \begin{align}
%     \theta^{\mathrm{MAP}} \defines \arg\max_{\theta} p(\theta \vbar \calD) = \arg\max_{\theta}  p(\calD \vbar \theta) p(\theta) ,
% \end{align}
% with prior distribution $p(\theta)$.
% Under the MAP estimate $\theta^\ast$, we obtain the MAP guidance function
% \begin{align*}
% \begin{split}
%     % &
%     \nabla \mathcal{S}^{\mathrm{MAP}}(\Xbf_{t})
%     % \\
%     &
%     =
%     \nabla \log p_{t}(\ybf \vbar \Xbf_{t}, \theta^{\mathrm{MAP}} ; f) + \nabla \log p_{t}(\Xbf_{t}) .
% \end{split}
% \end{align*}
% % A commonly used prior is an isotropic Gaussian distribution with \mbox{$p(\theta)=\calN(\theta;\mathbf{0},\lambda\mathbf{I})$}, which favors parameters with small $L_2$-norm.
% % While simple and useful, uninformative priors like this only reflect simple inductive biases and are unable to incorporate more sophisticated prior beliefs into model training, making them of limited use for problems in which encoding additional information can be critical.
% %for problems where additional information about the modeled domain is available.

% %While there is nothing particularly remarkable about this guidance function, its construction provides a blueprint for incorporating relevant task-specific information into the guidance function via informative data-driven priors.
% %We will discuss the construction of such priors and the construction of domain-informed guidance functions next.



% \subsection{Domain-Informed Guidance Functions}

% Next, we will build on this formulation to incorporate task-specific information into the guidance function by constructing a {\em domain-informed prior} that places high probability density on parameters that induce predictive models with desirable properties~\citep{rudner2023function}.

% %While it is challenging to construct data-independent informative priors over neural network parameters, we can use domain-specific data to construct informative {\em data-driven priors} that place high probability density on parameters that induce predictive models with desirable properties~\citep{rudner2023function}.

% Given labeled data $\calD$, domain-specific context data $\Hat{\calD}$, and a domain-informed data-driven prior $p(\theta \vbar \Hat{\calD})$, the posterior $p(\theta \vbar \calD, \Hat{\calD})$ reflects both the prior beliefs encoded in $p(\theta \vbar \Hat{\calD})$ as well as the information from the labeled data $\calD$.
% However, since computing $p(\theta \vbar \calD, \Hat{\calD})$ is intractable, we may instead, again, resort to using the MAP estimate,
% \begin{align}
% \label{eq:map_domain}
%     \hspace*{-5pt}\theta^\ast \defines \arg\max_{\theta} p(\theta \vbar \calD, \Hat{\calD}) = \arg\max_{\theta}  p(\calD \vbar \theta) p(\theta \vbar \Hat{\calD}) ,
% \end{align}
% which yields a tractable {\em domain-informed guidance function}
% \begin{align*}
% \begin{split}
% \label{eq:domain_informed_guidance}
%     % &
%     \mathcal{S}^{\ast}(\Xbf_{t})
%     % \\
%     &
%     =
%     \nabla \log p_{t}\left(\ybf \vbar \Xbf_{t}, \theta^{\ast} \right) + \nabla \log p_{t}(\Xbf_{t}) ,
% \end{split}
% \end{align*}
% which only differs from previous guidance function in the parameters $\theta^\ast$ in $q(\theta) \defines \delta(\theta - \theta^\ast)$.



\subsection{Domain-Informed Guidance Functions}

Explicitly including the guidance function parameterization in the SDE allows us to be more transparent about our modeling assumptions and reveals a broader design space for defining parametric guidance models.
If, for example, we want to incorporate task-specific information into the guidance function, we can specify \mbox{$q(\theta) \defines p(\theta \vbar \calD, \Hat{\calD})$}, where $p(\theta \vbar \calD)$ is the posterior distribution over the model parameters given labeled data $\calD = \{(\bx_{t}^{(n)},\ybf^{(n)})\}$ and $p(\theta \vbar \Hat{\calD})$ is a domain-informed prior.
Choosing the posterior \mbox{$p(\theta \vbar \calD)$} has an intuitive appeal:
It provides a probabilistically principled approach to incorporating information from labeled data into the guidance model and, via the domain-informed prior, allows encoding domain knowledge that can be leveraged when only little labeled data is available.

Unfortunately, computing $p(\theta \vbar \calD, \Hat{\calD})$ is not in general tractable, but instead of using the full posterior, we can use the {\em most likely parameters under the posterior} as a tractable alternative which---while not reflecting uncertainty about the model parameters---retains the ability to incorporate prior beliefs into the guidance model.
To use the most likely parameters under the posterior $p(\theta \vbar \calD, \Hat{\calD})$, we let $q(\theta) \defines \delta(\theta - \theta^\ast)$, where $\theta^\ast$ is the maximum a posteriori (\textsc{MAP}) estimate,
\begin{align}
\label{eq:map_domain}
    \hspace*{-5pt}\theta^\ast \defines \arg\max_{\theta} p(\theta \vbar \calD, \Hat{\calD}) = \arg\max_{\theta}  p(\calD \vbar \theta) p(\theta \vbar \Hat{\calD}) ,
\end{align}
which yields a tractable {\em domain-informed guidance function}
\begin{align}
\begin{split}
\label{eq:domain_informed_guidance}
    % &
    \mathcal{S}^{\ast}(\Xbf_{t})
    % \\
    &
    =
    \nabla \log p_{t}\left(\ybf \vbar \Xbf_{t}, \theta^{\ast} \right) + \nabla \log p_{t}(\Xbf_{t}) .
\end{split}
\end{align}


%While the construction of domain-informed guidance functions appears simple, the challenge in constructing them lies in defining a suitable data-driven prior used for MAP estimation (\Cref{eq:map_domain}).
%Next, we will show how to construct data-driven priors specifically designed for guided diffusion models and present a simple optimization objective for finding $\theta^\ast$.

%The challenge of constructing domain-informed guidance functions lies in defining a suitable data-driven prior used for MAP estimation (\Cref{eq:map_domain}).

% One such scenario is the optimization of parametric guidance models, where we often (i) have access to vast amounts of unlabeled data that span parts of the input space outside of the training domain and (ii) can specify desired properties of guidance functions on out-of-domain data points.
% % In the following, we build on prior work from \citet{rudner2023function} to construct a time-dependent probabilistic model that is able to integrate this additional information into the guidance model training process.
% % Specifically, we construct a regularization term that biases the model towards functions that fit the labeled data well and encode 
% In the next section, we will show how to construct and use data-driven domain-informed prior distributions when training guidance models.


\subsection{Training Domain-Informed Guidance Models}
\label{sec:training_robust_guidance_models}

To find $\theta^\ast \defines \arg\max_{\theta} p(\theta \vbar \calD, \Hat{\calD})$, we consider a standard supervised learning setting with $t=0,...,T$ and $N$ i.i.d. data realizations \mbox{${\calD_{t} = \{(\xbf_{t}^{(n)}, \by_{\calD}^{(n)})\}_{n=1}^{N}}$} of inputs \mbox{$\xbf_{t} \in \calX$} and targets \mbox{$\ybf \in \calY$}.
Furthermore, we define an observation model $\Bar{p}_{t}(\by_{\calD} \vbar \xbf_{t}, \theta; f)$ defined in terms of a guidance model
% $f(\cdot \,; \theta)$, with
\mbox{$f(\cdot \,; \theta) \defines \theta_{L}h(\cdot \,; \theta_{h})$} with \mbox{$h(\cdot \,; \theta_{h}):\calX\to\R^d$} and parameterized by parameters $\theta \defines \{ \theta_{h}, \theta_{L} \}$.
% , where $\theta_{h}$ are embedding parameters and $\theta_{L}$ are last-layer parameters.
% Furthermore, define an observation model $p_{\Ybf | \Xbf, \Theta}(\by_{\calD} \vbar \xbf_{t}, \theta; f)$ with a parametric mapping \mbox{$f(\cdot \,; \theta) \defines \theta_{L}h(\cdot \,; \theta_{h}):\calX\to\calY$} that generates a $d$-dimensional embedding \mbox{$h(\cdot \,; \theta_{h}):\calX\to\R^d$} and then applies an affine transformation \mbox{$\theta_{L}:\R^d\to\calY$}.

Conventional supervised learning techniques for training guidance models define a regularized timestep-dependent negative log-likelihood objective,
\begin{align*}
    \calL(\theta, \calD_{\mathcal{T}}, \mathcal{T})
    \defines
    -\sum_{n=1}^{N} \log{\Bar{p}_{\mathcal{T}}(\by^{(n)} \vbar \xbf^{(n)}_{\mathcal{T}} , \theta ; f)} + \frac{1}{2\lambda} ||\theta||_{2}^{2},
    % -\sum_{n=1}^{(n)} \log{p_{\Ybf | \Xbf, \Theta}(\by^{(n)} \vbar \xbf^{(n)}_{t} , \theta)}.
\end{align*}
where $\mathcal{T} \sim p_{\mathcal{T}}(t)$ is a random timestep, and optimize the parameters $\theta$ by minimizing the objective function
\begin{align}
\label{eq:standard_loss}
    \Bar{\calL}(\theta, \calD_{\mathcal{T}}, \mathcal{T})
    \defines
    \E_{p_{\mathcal{T}}}\left[ \calL(\theta, \calD_{\mathcal{T}}, \mathcal{T}) \right] .
\end{align}
However, when labeled data is biased and scarce, the objective in~\Cref{eq:standard_loss} may lead to predictive models that do not generalize well outside of their training domain \citep{ovadia2019can,koh2021wilds} and perform poorly under noise perturbations \cite{szegedy2013intriguing,goodfellow2014explaining,ho2022classifier}.

To improve the reliability of models in this setting, we consider a family of domain-informed priors $p(\theta \vbar \Hat{\calD})$ that favor solutions that exhibit a desirable behavior \mbox{$\Hat{\ybf}\subseteq\calY^M$} on a problem-specific out-of-distribution context set $\Hat{\xbf} \defines \{ \Hat{\xbf}_{t} \}_{t=0}^{T}$ with \mbox{$\Hat{\xbf}_{t}\subseteq\calX^M$}~\citep{rudner2022tractable,rudner2023function}.
% While the desired behavior on out-of-distribution data points is often application-dependent, we find that encouraging uncertain predictions in areas of the input domain with little or no signal from the supervised learning process performs well across settings.
% This \emph{Gaussian process prior} minimizes overconfident predictions and allows the conditional denoising process to focus on near out-of-distribution regions with the highest likelihood of containing molecules with improved properties.
While the specific choice of $\Hat{\ybf}$ is application-dependent, 
%of predictive models evaluated on out-of-distribution data 
we can construct a broadly applicable prior that places high probability density on parameter values that induce models with high predictive uncertainty on the context set that increases as a function of the timestep $t$.

To do so, we build on the result in \citet{rudner2023function}, which showed that MAP estimation with domain-informed priors, which can be expressed as $p(\theta \vbar \Hat{\calD}) = \frac{\Hat{p}(\Hat{\ybf} \vbar \Hat{\xbf}, \theta) \Hat{p}(\theta)}{\Hat{p}(\Hat{\ybf} \vbar \Hat{\xbf})}$ by Bayes theorem, only requires specifying a tractable joint distribution $\Hat{p}(\Hat{\ybf} \vbar \Hat{\xbf}, \theta) \Hat{p}(\theta)$.

To construct a domain-informed auxiliary likelihood function $\Hat{p}(\Hat{\ybf} \vbar \Hat{\xbf}, \theta)$, we extend the prior presented in \citet{rudner2023function}.
First, we use a fixed set of parameters $\phi$ (either randomly initialized or pre-trained), to obtain embeddings \mbox{$\Hat{\Hbf}_{t} = h(\Hat{\xbf}_{t}, \phi)\in\R^{M\times d}$}, evaluated at a set of $M$ context points.
We then leverage the inner product of context points in this embedding space to regularize the smoothness of the functions learned by our guidance model through the covariance matrix
\begin{align}
\begin{split}
    \mathbf{K}_{t}(\Hat{\Hbf}_{t}, t) = \sigma_{t} \Hat{\Hbf}_{t}\Hat{\Hbf}_{t}^T+\tau_{t}\mathbf{I},
\end{split}
\end{align}
where the covariance scale $\sigma_{t}$ determines how strongly predictions can vary between similar context points and the diagonal scale $\tau_{t}$ specifies how closely the predictions should match the desired outputs $\Hat{\ybf}$.
% In classification settings, $\Hat{\ybf}_{t}$ is given by a zero-logit vector 
%$\Hat{\ybf}=\mathbf{0}$ 
% that encourages equal class probabilities.
Unfortunately, \citet{rudner2023function} only considered data-driven priors for classification settings.
To construct a data-driven prior that leads to more reliable uncertainty in regression settings where the learned predictive model consists of a learned mean function and a learned variance function, we define $\Hat{\ybf}_{1} \defines \frac{1}{N}\sum_{n=1}^{N} y^{(n)}$ and $\Hat{\ybf}_{2} \defines \boldsymbol{\sigma_{0}}$, a variance hyperparameter.
Putting everything together, we can show that
\begin{align*}
    &
    \log p(\theta \vbar \Hat{\calD})
    \\
    &
    \propto
    \log \prod_{i=1,2 }\calN([f(\hat{\xbf}_{t} ; \theta)]_{i} ; \Hat{\ybf}_{i}, \mathbf{K}_{t}(\Hat{\Hbf}_{t}, t)) + \frac{1}{2\lambda}\|\theta\|_{2}^{2} ,
\end{align*}
where $[f(\hat{\xbf}_{t} ; \theta)]_{1}$ and $[f(\hat{\xbf}_{t} ; \theta)]_{2}$ denote the mean and the variance output of the guidance model, respectively.
Intuitively, this prior can be viewed as enforcing smoothness constraints via a Gaussian process with a product kernel.
% Since having a well-calibrated predictive model is particularly important in the earlier stages of the sample generation process (i.e., for small $t$), we need to construct a data-driven prior that takes the noise level $\beta_t$ into account.
% The full regularizer is given by the negative log-likelihood of a multivariate Gaussian distribution with mean $\ybf$ and covariance $\mathbf{K}_{t}(\Hat{\Hbf}_{t}, t)$
To relate this log prior to more conventional training techniques, we note that we can view MAP estimation with a data-driven prior as maximum likelihood estimation with a domain-informed regularizer
\begin{align*}
\begin{split}
    &
    R^\ast_{t}(\theta, f, \hat{\xbf}_{t}, t)
    % \\
    % &
    % \defines
    % \E_{p_{T}}\left[ \log p(\theta \vbar \Hat{\calD}, T) \right]
    % \\
    % &
    =
    - \log \prod_{i=1,2} \calN([f(\hat{\xbf}_{t}]_{i} ; \theta) ; \Hat{\ybf},\mathbf{K}_{t}(\Hat{\Hbf}_{t}, t))
    % \\
    % &
    % =
    % \sum_{k = 1}^{K} \frac{\tau_{f}}{2} d^{2}_{M}(f(\hat{\xbf}_{T} ; \theta)_{k},  \mathbf{K}_{t}(\Hat{\Hbf}_{t}, t)
    % \hspace*{-2pt}-\hspace*{-2pt} 
    % \frac{\tau_{\theta}}{2} \|\theta\|_{2}^{2} ,
    % \hspace*{-2pt}-\hspace*{-2pt}
    % \E_{p_{T}}\left[ \sum_{k = 1}^{K} \frac{\tau_{f}}{2} d^{2}_{M}(f(\hat{\xbf}_{T} ; \theta)_{k}, K(\hat{\xbf}_{T}, \hat{\xbf}_{T} ; \phi_{0})) \right] 
    % \hspace*{-2pt}-\hspace*{-2pt} 
    % \frac{\tau_{\theta}}{2} \|\theta\|_{2}^{2} ,
\end{split}
\end{align*}
% \begin{align}
%     R(\theta, f, \hat{\xbf})
%     \defines
%     \hspace*{-2pt}-\hspace*{-2pt}
%     \frac{\tau_{f}}{2} d^{2}_{M}(f(\hat{\xbf}_{t} ; \theta)_{k}, K(\hat{\xbf}_{t}, \hat{\xbf}_{t} ; \phi)) ,
% \end{align}
At each training step, a mini-batch is sampled from the context set and perturbed with the same noising process as the unconditional diffusion model.
To avoid overconfident predictions as context points approach the invariant distribution $\calN(\mathbf{0},\mathbf{I})$, we increase $\tau_{t}$ with the same schedule as the noise scales $\beta_t$.
Similarly, as the distinction between in- and out-of-distribution points becomes meaningless at larger noise levels, we decrease $\sigma_{t}$ with an inverted schedule.

Combining this approach with an additional $L_2$ regularization term and the supervised loss from \Cref{eq:standard_loss}, we arrive at the modified training objective
\begin{align}
\label{eq:fseb_loss}
\begin{split}
    % &
    % \hspace{-7pt}
    \mathcal{L}^\ast(\theta, \calD, \hat{\xbf})
    % \\
    % &
    % \hspace{-4pt}
    =
    % \hspace*{-2pt}
    \E_{p_{\mathcal{T}}}[ \calL(\theta, \calD_{\mathcal{T}}, \mathcal{T})] + \E_{p_{\mathcal{T}}}[ R^\ast_{\mathcal{T}}(\theta, f, \hat{\xbf}_{\mathcal{T}}, \mathcal{T}) ]
    % \hspace*{-2pt}\E_{p_T}\left[\calL(\xbf^{\calD}_0, \by^{\calD}, \theta, t) + \Hat{R}_{t}(\theta, f, \hat{\xbf}_{t}, t)\right] 
    %\\
    %&
    % + \frac{1}{2\lambda}\|\theta\|_{2}^{2} .
    % \nonumber 
\end{split}
\end{align}
As shown in \citet{rudner2023function}, optimizing this objective corresponds to MAP estimation with a data-driven prior as shown in \Cref{eq:map_domain}.
Finally, using the learned parameters $\theta^\ast$ as shown in \Cref{eq:domain_informed_guidance} allows us to perform domain-informed guided diffusion.


% where \mbox{$d^{2}_{M}(v, K) \defines v^\top K^{-1} v$} is the squared Mahalanobis distance between $v$ and $\mathbf{0}$.


%\textcolor{red}{Why these are simple to compute and scalable.Why is this ``domain informed''. Why encourage uncertainty? Cite QSAVI.}



%This approach allows us to encode domain-informed prior knowledge through both the form of the  functional prior and the set of context points that we enforce it on. 

% \subsection{Domain-Informed Guidance Models as Bayesian Inference}


%\textcolor{red!50!black}{TO DO}


% ------------ PRIOR TEXT ------------

% Consider the standard supervised learning setting with $N$ i.i.d. data realizations \mbox{${\calD = \{\xbf^{(n)}_0, \by^{(n)}\}_{n=1}^{(n)}} = (\xbf^\calD_0, \mathbf{y}^\calD)$} of inputs \mbox{$\xbf_{t} \in \calX$} and targets \mbox{$\Ybf \in \calY$} with input space \mbox{$\calX \subseteq \real^D$} and target space \mbox{$\calY \subseteq \real^K$} for regression and \mbox{$\calY \subseteq \{0, 1\}^K$} for classification tasks with $K$ classes.
% Further, define a parametric observation model $p_{\Ybf | \Xbf, \Theta}(\by \vbar \xbf, \theta; f)$ with mapping \mbox{$f(\cdot \,; \theta) \defines h(\cdot \,; \theta_{h}) \theta_{L}$}.

% Conventional supervised learning training routines involve minimization of the negative log-likelihood objective function
% \begin{align*}
% % \label{eq:map}
%     \calL(\theta, \xbf_{\calD}, \by_{\calD})
%     =
%     -\sum_{n=1}^{(n)} \log{p_{\Ybf | \Xbf, \Theta}(\by^{(n)}_{\calD} \vbar \xbf^{(n)}_{\calD} , \theta)}
% \end{align*}
% with respect to $\theta$.

% To learn models that exhibit improved generalization under covariate shifts and have well-calibrated predictive uncertainty estimates, we consider training with a domain-informed regularizer $R(\theta, f, \hat{\xbf})$ that favors solutions that induce predictive functions with high predictive uncertainty on a domain-specific set of input points $\hat{\xbf}$.
% The resulting optimization objective is given by
% \begin{align*}
%     &
%     \calF(\theta, \xbf_{\calD}, \by_{\calD})
%     \\
%     % ~
%     &
%     =
%     \E_{q_{\varepsilon}}\bigg[
%     -\sum_{n=1}^{(n)} \log{p_{\Ybf | \Xbf, \Theta}(\by^{(n)}_{\calD} \vbar \xbf^{(n)}_{\calD} , \theta + \varepsilon)} + R(\theta, f, \hat{\xbf}) \bigg] ,
% \end{align*}
% where $\varepsilon \sim \calN(\varepsilon ; 0, \gamma)$ for some fixed, small $\gamma$ (e.g., $\gamma = 10^{-10}$).

% The specific functional form of the regularizer depends on the prediction problem.
% For classification tasks, we consider the negative squared Mahalanobis distance penalty proposed in \citet{rudner2023function}:
% \begin{align}
%     R(\theta, f, \hat{\xbf})
%     \defines
%     \hspace*{-2pt}-\hspace*{-2pt}
%     \sum_{k = 1}^{K} \frac{\tau_{f}}{2} d^{2}_{M}(f(\hat{\xbf} ; \theta)_{k}, K(\hat{\xbf}, \hat{\xbf} ; \phi_{0})) 
%     \hspace*{-2pt}-\hspace*{-2pt} 
%     \frac{\tau_{\theta}}{2} \|\theta\|_{2}^{2} ,
% \end{align}
% where \mbox{$d^{2}_{M}(v, K) \defines v^\top K^{-1} v$} is the squared Mahalanobis distance between $v$ and $\mathbf{0}$.
% For regression tasks, we consider
% % \begin{align}
% %     XXX .
% % \end{align}

%\subsection{Domain-Aware Guidance as Posterior Predictive Gradient Marginalization}

% \TR{
% \begin{itemize}
%     \item
%     Show that we can view gradient in guidance as gradient of the likelihood under the mode the parameter posterior (conditioned on training data and context data)
%     \item
%     Show that guidance update follows exactly from Gaussian marginalization
% \end{itemize}
% }

% To provide an intuition for domain-informed guidance, we show that we can frame the sampling process as marginalization over the gradients of a Bayesian posterior predictive distribution.
% To do so, first, we note that the training neural networks using the regularized objective in \Cref{xxx} corresponds to approximating a posterior distribution over neural network parameters, $p(\theta \vbar \calD, \hat{\calD})$, where \mbox{${\hat{\calD} = \{\hat{\xbf}^{(m)}, \hat{\by}^{(m)}\}_{m=1}^M} = (\hat{\xbf}, \hat{\by})$}.

% Next, we note that guided diffusion can be viewed as marginalization over gradients of a specific loss function:
% \begin{align}
% \begin{split}
%     % &
%     p(\xbf_{t-1} \vbar \xbf_{t})
%     % \\
%     &
%     =
%     \int p(\xbf_{t-1} \vbar \xbf_{t}, \mathbf{z}_{t}) p(\mathbf{z}_{t}) \,\dee \mathbf{z}_{t}
%     \\
%     &
%     =
%     \int \calN(\xbf_{t-1} ; \bmu_{t}(\xbf_{t}) + \bSigma_{t} \mathbf{z}_{t} , \sqrt{\alpha} \bSigma_{t})
%     \\
%     &
%     \qquad~~
%     \cdot \calN(\mathbf{z}_{t} ; \mathbf{g}_{t}(\xbf_{t},\ybf), \gamma \Sigma^{-1} ) \,\dee \mathbf{z}_{t}
%     \\
%     &
%     =
%     \calN(\xbf_{t-1} ; \bmu_{t} + \bSigma_{t}\mathbf{g}_{t}(\xbf_{t},\ybf), \bSigma_{t}) ,
% \end{split}
% \end{align}
% where $\gamma = \frac{1 - \sqrt{\alpha}}{\alpha}$ for $0 < \alpha < 1$, and $\mathbf{g}_{t}(\xbf_{t},\ybf)$ is as defined before.
% This is the standard guided diffusion distribution, but this derivation does not require any first-order approximations.
% Finally, instead of using the gradient of a conventionally trained---deterministic---guidance model, we consider the gradient with respect to $\xbf$ under the {\em expected} negative log-likelihood, where the expectation is computed under a Bayesian posterior distribution over the neural network parameters, that is,
% \begin{align}
%     \mathbf{g}^{\mathrm{Bayes}}(\xbf_{t},\ybf)
%     =
%     \nabla_{\xbf} \E_{p_{\Theta | \calD, \hat{\calD}}}[\calL(\Theta, \xbf, \by)]|_{\xbf=\xbf_{t}} .
% \end{align}
% Since computing $p(\theta \vbar \calD, \hat{\calD})$ is not in general tractable, we need to approximate the posterior.
% By minimizing $\calF(\theta, \xbf_{\calD}, \by_{\calD})$ in \Cref{xxx} with respect to $\theta$, we obtain such an approximation.

% Domain-aware guidance using these parameters is then given by
% \begin{align}
%     \calN(\xbf_{t-1} ; \bmu_{t} + \bSigma_{t}\hat{\mathbf{g}}^{q}_{t}(\xbf_{t},\ybf), \bSigma_{t})
% \end{align}
% with the unbiased Monte Carlo gradient estimate
% \begin{align}
%     \hat{\mathbf{g}}^{q}(\xbf_{t},\ybf)
%     =
%     \frac{1}{S} \sum_{s = 1}^{s} \nabla_{\xbf} \calL(\theta + \varepsilon^{(s)}, \xbf, \by) ]|_{\xbf = \xbf_{t}} ,
% \end{align}
% where $\varepsilon^{(s)} \sim \calN(\varepsilon ; 0, \gamma)$




% By favoring posterior distributions $p_{\Theta\vert\calD}$ that are able to reconcile the signal from a small, labeled dataset with pre-specified modeling preferences, our method biases the training of this guidance model towards functions that are likely to perform well across larger subsets of the input domain.

% Since computing $p(\theta \vbar \calD, \hat{\calD})$ is not in general tractable, we need to approximate the posterior.
% By minimizing $\calF(\theta, \xbf_{\calD}, \by_{\calD})$ in \Cref{xxx} with respect to $\theta$, we obtain such an approximation.

% Domain-aware guidance using these parameters is then given by
% \begin{align}
%     \calN(\xbf_{t-1} ; \bmu_{t} + \bSigma_{t}\hat{\mathbf{g}}^{q}_{t}(\xbf_{t},\ybf), 2 \bSigma_{t})
% \end{align}
% with the unbiased Monte Carlo gradient estimate
% \begin{align}
%     \hat{\mathbf{g}}^{q}(\xbf_{t},\ybf)
%     =
%     \frac{1}{S} \sum_{s = 1}^{s} \nabla_{\xbf} \calL(\theta + \varepsilon^{(s)}, \xbf, \by) ]|_{\xbf = \xbf_{t}} ,
% \end{align}
% where $\varepsilon^{(s)} \sim \calN(\varepsilon ; 0, \gamma)$


% To do so, first, we note that the training neural networks using the regularized objective in \Cref{xxx} corresponds to approximating a posterior distribution over neural network parameters, $p(\theta \vbar \calD, \hat{\calD})$, where \mbox{${\hat{\calD} = \{\hat{\xbf}^{(m)}, \hat{\by}^{(m)}\}_{m=1}^M} = (\hat{\xbf}, \hat{\by})$}.

% When using guidance in diffusion models, the goal is to generate samples that are representative of the training distribution and yet novel.
% Standard guidance functions used in the literature, do not necessarily have the ability to enable generation of such samples.
% This is because, in order to generate samples that reflect properties of the training distribution, but are also meaningfully different, guidance functions need to be able to generalize under covariate shifts.
% That is, in order for guidance functions to encourage the generation of samples that are meaningfully different from samples in the training distribution, the guidance function needs to place high probability density on samples that are related to the training data while also being meaningfully different.
% Neural networks trained with standard supervised learning routines have been shown to generalize poorly under covariate shifts, meaning that they do not provide a good model for recognizing related but meaningfully distinct points in input space.
% This shortcoming creates a problem for classifier guidance in diffusion models.
% In order for guidance functions in diffusion models to meaningfully improve generation, they need to be able to extract a meaningful signal from noisy input points and generalize distribution shifts.

% We propose a simple regularizer that can be used to train classifiers that lead to significantly improved guidance functions.
% We then show that this simple addition to standard supervised learning routines can be viewed as performing approximate Bayesian inference with a domain-informed data-driven prior over the neural network parameters.

% \TR{
% \begin{itemize}
%     \item
%     Outline what kinds of properties we need in guidance functions
%     \item
%     Show how to train a model that has the desired properties
%     \begin{itemize}
%         \item
%         Show that training just requires additional regularizer (show for regression and classification, which require different priors)
%         \item 
%         Show how to use a plug-and-play regularizer
%     \end{itemize}
% \end{itemize}
% }



==> include/aabi/custom_aabi2023.tex <==
%%%%%%% LAYOUT

% \usepackage[
%   paper  = letterpaper,
%   left   = 1.65in,
%   right  = 1.65in,
%   top    = 1.0in,
%   bottom = 1.0in,
%   ]{geometry}
% Set the typeface to Times Roman
% \usepackage{times}
% Changes typeface to Bitstream Charter
% \usepackage[bitstream-charter]{mathdesign}
% \usepackage{include/jmlr2e}


\usepackage{titletoc}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{colortbl}

\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut


\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}

\newtheorem{innercustomassumption}{Assumption}
\newenvironment{customassumption}[1]
  {\renewcommand\theinnercustomassumption{#1}\innercustomassumption}
  {\endinnercustomassumption}
  
% \newcommand\defines{\stackrel{\mathclap{\normalfont\mbox{\tiny def}}}{=}}
\newcommand\defines{\,\dot{=}\,}

\newcommand{\ntk}{\textsc{ntk}\xspace}
\newcommand{\map}{\textsc{map}\xspace}
\newcommand{\fsmap}{\textsc{fsmap}\xspace}
\newcommand{\rmfvi}{\textsc{mfvi-radial}\xspace}
\newcommand{\tmfvi}{\textsc{mfvi-tempered}\xspace}
\newcommand{\swag}{\textsc{swag}\xspace}
\newcommand{\mcd}{\textsc{mc dropout}\xspace}
\newcommand{\vcl}{\textsc{vcl}\xspace}


\newcommand{\vbar}{\,|\,}


\newcommand{\bThetahat}{\smash{\hat{\bTheta}}}
\newcommand{\bthetahat}{\smash{\hat{\btheta}}}
\newcommand{\flin}{\smash{\hat{f}}}



\newcommand{\jac}{\mathcal{J}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calC}{\mathcal{C}}

\newcommand{\DD}{\mathbb{D}}

\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\biota}{\boldsymbol{\iota}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}

\newcommand{\qtilde}{\smash{\tilde{q}}}
\newcommand{\ptilde}{\smash{\tilde{p}}}

\newcommand{\bxhat}{\hat{\mathbf{x}}}
\newcommand{\bXhat}{\hat{\mathbf{X}}}
\newcommand{\byhat}{\hat{\mathbf{y}}}
\newcommand{\bYhat}{\hat{\mathbf{Y}}}

\newcommand{\bxbar}{\bar{\mathbf{x}}}
\newcommand{\bXbar}{\bar{\mathbf{X}}}
\newcommand{\bybar}{\bar{\mathbf{y}}}
\newcommand{\bYbar}{\bar{\mathbf{Y}}}






\newcommand{\pms}[1]{\ensuremath{{\scriptstyle\pm #1}}}


\usepackage{standalone}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgf}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
\usetikzlibrary{angles,quotes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{fit}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{shadings}
\usetikzlibrary{shapes}
\usetikzlibrary{fadings}
\usetikzlibrary{bayesnet}
\usetikzlibrary{matrix}
\usetikzlibrary{plotmarks}
\usetikzlibrary{intersections}
\usetikzlibrary{pgfplots.fillbetween}
\pgfplotsset{compat=1.14}
%
\usepackage{siunitx}

\usepackage{colortbl}
\definecolor{mediumgray}{gray}{0.7}
\definecolor{lightgray}{gray}{0.85}
\definecolor{lightlightgray}{gray}{0.9}
\definecolor{C1}{HTML}{1F77B4}
\definecolor{C2}{HTML}{FF7F0E}
\definecolor{C3}{HTML}{2CA02C}
\definecolor{C4}{HTML}{D62728}
\definecolor{C5}{HTML}{9467BD}
\colorlet{C1light}{C1!70!white}
\colorlet{C2light}{C2!70!white}
\colorlet{C3light}{C3!70!white}
\colorlet{C4light}{C4!70!white}
\colorlet{C5light}{C5!70!white}
\colorlet{C1lighter}{C1!50!white}
\colorlet{C2lighter}{C2!50!white}
\colorlet{C3lighter}{C3!50!white}
\colorlet{C4lighter}{C4!50!white}
\colorlet{C5lighter}{C5!50!white}
\colorlet{C1vlight}{C1!20!white}
\colorlet{C2vlight}{C2!20!white}
\colorlet{C3vlight}{C3!20!white}
\colorlet{C4vlight}{C4!20!white}
\colorlet{C5vlight}{C5!20!white}
\colorlet{linkcolor}{violet}
% \colorlet{citecolor}{RedOrange}  %
% \colorlet{urlcolor}{Aquamarine}

\newtheorem{approximation}{Approximation}

%%%%%%% TEXT ACRONYMS

\newcommand{\dgps}{\textsc{dgp}s\xspace}
\newcommand{\dgp}{\textsc{dgp}\xspace}
\newcommand{\gps}{\textsc{gp}s\xspace}
\newcommand{\gp}{\textsc{gp}\xspace}
\newcommand{\bnn}{\textsc{bnn}\xspace}
\newcommand{\bnns}{\textsc{bnn}s\xspace}
\newcommand{\np}{\textsc{np}\xspace}
\newcommand{\nps}{\textsc{np}s\xspace}
\newcommand{\vae}{\textsc{vae}\xspace}
\newcommand{\vaes}{\textsc{vae}s\xspace}
\newcommand{\iwvae}{\textsc{iwvae}\xspace}
\newcommand{\iwvaes}{\textsc{iwvae}s\xspace}
\newcommand{\vi}{\textsc{vi}\xspace}
\newcommand{\svi}{\textsc{svi}\xspace}
\newcommand{\dsvi}{\textsc{dsvi}\xspace}
\newcommand{\fsvi}{\textsc{fsvi}\xspace}
\newcommand{\psvi}{\textsc{psvi}\xspace}
\newcommand{\iwvi}{\textsc{iwvi}\xspace}
\newcommand{\snr}{\textsc{snr}\xspace}
\newcommand{\snrs}{\textsc{snr}s\xspace}
\newcommand{\dreg}{\textsc{dreg}\xspace}
\newcommand{\clt}{\textsc{clt}\xspace}
\newcommand{\elbo}{\textsc{elbo}\xspace}
\newcommand{\elbos}{\textsc{elbo}s\xspace}
\newcommand{\kld}{KL divergence\xspace}
\newcommand{\fsgc}{\textsc{fsgc}\xspace}
\newcommand{\psmap}{\textsc{ps-map}\xspace}
\newcommand{\jsd}{JS divergence}



\usepackage{tcolorbox}

\newcommand{\hypothesis}[2]{%
\begin{tcolorbox}[colback=blue!10!white,leftrule=2.5mm,size=title]
\textbf{#1}: #2
\end{tcolorbox}
\vspace{-0.1cm}%
}

==> include/aistats/custom_aistats2024.tex <==
%%%%%%% LAYOUT

% \usepackage[
%   paper  = letterpaper,
%   left   = 1.65in,
%   right  = 1.65in,
%   top    = 1.0in,
%   bottom = 1.0in,
%   ]{geometry}
% Set the typeface to Times Roman
% \usepackage{times}
% Changes typeface to Bitstream Charter
% \usepackage[bitstream-charter]{mathdesign}
% \usepackage{include/jmlr2e}


\usepackage{titletoc}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{colortbl}

\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut


\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}

\newtheorem{innercustomassumption}{Assumption}
\newenvironment{customassumption}[1]
  {\renewcommand\theinnercustomassumption{#1}\innercustomassumption}
  {\endinnercustomassumption}
  
% \newcommand\defines{\stackrel{\mathclap{\normalfont\mbox{\tiny def}}}{=}}
\newcommand\defines{\,\dot{=}\,}

\newcommand{\ntk}{\textsc{ntk}\xspace}
\newcommand{\map}{\textsc{map}\xspace}
\newcommand{\rmfvi}{\textsc{mfvi-radial}\xspace}
\newcommand{\tmfvi}{\textsc{mfvi-tempered}\xspace}
\newcommand{\swag}{\textsc{swag}\xspace}
\newcommand{\mcd}{\textsc{mc dropout}\xspace}
\newcommand{\vcl}{\textsc{vcl}\xspace}


\newcommand{\vbar}{\,|\,}


\newcommand{\bThetahat}{\smash{\hat{\bTheta}}}
\newcommand{\bthetahat}{\smash{\hat{\btheta}}}
\newcommand{\flin}{\smash{\hat{f}}}



\newcommand{\jac}{\mathcal{J}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calC}{\mathcal{C}}

\newcommand{\DD}{\mathbb{D}}

\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\biota}{\boldsymbol{\iota}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}

\newcommand{\qtilde}{\smash{\tilde{q}}}
\newcommand{\ptilde}{\smash{\tilde{p}}}


\newcommand{\pms}[1]{\ensuremath{{\scriptstyle\pm #1}}}


\usepackage{standalone}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgf}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
\usetikzlibrary{angles,quotes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{fit}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{shadings}
\usetikzlibrary{shapes}
\usetikzlibrary{fadings}
\usetikzlibrary{bayesnet}
\usetikzlibrary{matrix}
\usetikzlibrary{plotmarks}
\usetikzlibrary{intersections}
\usetikzlibrary{pgfplots.fillbetween}
\pgfplotsset{compat=1.14}
%
\usepackage{siunitx}

\usepackage{colortbl}
\definecolor{mediumgray}{gray}{0.7}
\definecolor{lightgray}{gray}{0.85}
\definecolor{lightlightgray}{gray}{0.9}
\definecolor{C1}{HTML}{1F77B4}
\definecolor{C2}{HTML}{FF7F0E}
\definecolor{C3}{HTML}{2CA02C}
\definecolor{C4}{HTML}{D62728}
\definecolor{C5}{HTML}{9467BD}
\colorlet{C1light}{C1!70!white}
\colorlet{C2light}{C2!70!white}
\colorlet{C3light}{C3!70!white}
\colorlet{C4light}{C4!70!white}
\colorlet{C5light}{C5!70!white}
\colorlet{C1lighter}{C1!50!white}
\colorlet{C2lighter}{C2!50!white}
\colorlet{C3lighter}{C3!50!white}
\colorlet{C4lighter}{C4!50!white}
\colorlet{C5lighter}{C5!50!white}
\colorlet{C1vlight}{C1!20!white}
\colorlet{C2vlight}{C2!20!white}
\colorlet{C3vlight}{C3!20!white}
\colorlet{C4vlight}{C4!20!white}
\colorlet{C5vlight}{C5!20!white}
\colorlet{linkcolor}{violet}
% \colorlet{citecolor}{RedOrange}  %
% \colorlet{urlcolor}{Aquamarine}

\newtheorem{approximation}{Approximation}

\newcommand{\psvi}{\textsc{psvi}\xspace}


==> include/comments.tex <==
\newcommand{\tim}[1]{\xxcomment{blue}{T}{R}{#1}}
\newcommand{\sanae}[1]{\xxcomment{green}{S}{L}{#1}}
\newcommand{\andrew}[1]{\xxcomment{green}{A}{W}{#1}}
\newcommand{\marco}[1]{\xxcomment{green}{M}{M}{#1}}
\newcommand{\julia}[1]{\xxcomment{green}{J}{K}{#1}}
\newcommand{\brandon}[1]{\xxcomment{green}{B}{A}{#1}}
\newcommand{\lily}[1]{\xxcomment{green}{L}{L}{#1}}
\newcommand{\nate}[1]{\xxcomment{green}{N}{G}{#1}}
\newcommand{\shikai}[1]{\xxcomment{green}{S}{Q}{#1}}
\newcommand{\sanyam}[1]{\xxcomment{green}{S}{K}{#1}}




==> include/neurips/custom_neurips2023.tex <==
%%%%%%% LAYOUT

% \usepackage[
%   paper  = letterpaper,
%   left   = 1.65in,
%   right  = 1.65in,
%   top    = 1.0in,
%   bottom = 1.0in,
%   ]{geometry}
% Set the typeface to Times Roman
% \usepackage{times}
% Changes typeface to Bitstream Charter
% \usepackage[bitstream-charter]{mathdesign}
% \usepackage{include/jmlr2e}


\usepackage{titletoc}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{colortbl}

\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut


\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}

\newtheorem{innercustomassumption}{Assumption}
\newenvironment{customassumption}[1]
  {\renewcommand\theinnercustomassumption{#1}\innercustomassumption}
  {\endinnercustomassumption}
  
% \newcommand\defines{\stackrel{\mathclap{\normalfont\mbox{\tiny def}}}{=}}
\newcommand\defines{\,\dot{=}\,}

\newcommand{\ntk}{\textsc{ntk}\xspace}
\newcommand{\map}{\textsc{map}\xspace}
\newcommand{\rmfvi}{\textsc{mfvi-radial}\xspace}
\newcommand{\tmfvi}{\textsc{mfvi-tempered}\xspace}
\newcommand{\swag}{\textsc{swag}\xspace}
\newcommand{\mcd}{\textsc{mc dropout}\xspace}
\newcommand{\vcl}{\textsc{vcl}\xspace}


\newcommand{\vbar}{\,|\,}


\newcommand{\bThetahat}{\smash{\hat{\bTheta}}}
\newcommand{\bthetahat}{\smash{\hat{\btheta}}}
\newcommand{\flin}{\smash{\hat{f}}}



\newcommand{\jac}{\mathcal{J}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calC}{\mathcal{C}}

\newcommand{\DD}{\mathbb{D}}

\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\biota}{\boldsymbol{\iota}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}

\newcommand{\qtilde}{\smash{\tilde{q}}}
\newcommand{\ptilde}{\smash{\tilde{p}}}


\newcommand{\pms}[1]{\ensuremath{{\scriptstyle\pm #1}}}


\usepackage{standalone}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgf}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
\usetikzlibrary{angles,quotes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{fit}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{shadings}
\usetikzlibrary{shapes}
\usetikzlibrary{fadings}
\usetikzlibrary{bayesnet}
\usetikzlibrary{matrix}
\usetikzlibrary{plotmarks}
\usetikzlibrary{intersections}
\usetikzlibrary{pgfplots.fillbetween}
\pgfplotsset{compat=1.14}
%
\usepackage{siunitx}

\usepackage{colortbl}
\definecolor{mediumgray}{gray}{0.7}
\definecolor{lightgray}{gray}{0.85}
\definecolor{lightlightgray}{gray}{0.9}
\definecolor{C1}{HTML}{1F77B4}
\definecolor{C2}{HTML}{FF7F0E}
\definecolor{C3}{HTML}{2CA02C}
\definecolor{C4}{HTML}{D62728}
\definecolor{C5}{HTML}{9467BD}
\colorlet{C1light}{C1!70!white}
\colorlet{C2light}{C2!70!white}
\colorlet{C3light}{C3!70!white}
\colorlet{C4light}{C4!70!white}
\colorlet{C5light}{C5!70!white}
\colorlet{C1lighter}{C1!50!white}
\colorlet{C2lighter}{C2!50!white}
\colorlet{C3lighter}{C3!50!white}
\colorlet{C4lighter}{C4!50!white}
\colorlet{C5lighter}{C5!50!white}
\colorlet{C1vlight}{C1!20!white}
\colorlet{C2vlight}{C2!20!white}
\colorlet{C3vlight}{C3!20!white}
\colorlet{C4vlight}{C4!20!white}
\colorlet{C5vlight}{C5!20!white}
\colorlet{linkcolor}{violet}
% \colorlet{citecolor}{RedOrange}  %
% \colorlet{urlcolor}{Aquamarine}

\newtheorem{approximation}{Approximation}

\newcommand{\psvi}{\textsc{psvi}\xspace}


==> include/note/custom_note.tex <==
%%%%%%% LAYOUT

% \usepackage[
%   paper  = letterpaper,
%   left   = 1.65in,
%   right  = 1.65in,
%   top    = 1.0in,
%   bottom = 1.0in,
%   ]{geometry}
% Set the typeface to Times Roman
% \usepackage{times}
% Changes typeface to Bitstream Charter
% \usepackage[bitstream-charter]{mathdesign}
% \usepackage{include/jmlr2e}


\usepackage{titletoc}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{colortbl}

\newcommand\Tstrut{\rule{0pt}{2.6ex}}         % = `top' strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}}   % = `bottom' strut


\definecolor{azure}{rgb}{0.0, 0.5, 1.0}
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}

\newtheorem{innercustomassumption}{Assumption}
\newenvironment{customassumption}[1]
  {\renewcommand\theinnercustomassumption{#1}\innercustomassumption}
  {\endinnercustomassumption}
  
% \newcommand\defines{\stackrel{\mathclap{\normalfont\mbox{\tiny def}}}{=}}
\newcommand\defines{\,\dot{=}\,}

\newcommand{\ntk}{\textsc{ntk}\xspace}
\newcommand{\map}{\textsc{map}\xspace}
\newcommand{\fsmap}{\textsc{fsmap}\xspace}
\newcommand{\rmfvi}{\textsc{mfvi-radial}\xspace}
\newcommand{\tmfvi}{\textsc{mfvi-tempered}\xspace}
\newcommand{\swag}{\textsc{swag}\xspace}
\newcommand{\mcd}{\textsc{mc dropout}\xspace}
\newcommand{\vcl}{\textsc{vcl}\xspace}


\newcommand{\vbar}{\,|\,}


\newcommand{\bThetahat}{\smash{\hat{\bTheta}}}
\newcommand{\bthetahat}{\smash{\hat{\btheta}}}
\newcommand{\flin}{\smash{\hat{f}}}



\newcommand{\jac}{\mathcal{J}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calC}{\mathcal{C}}

\newcommand{\DD}{\mathbb{D}}

\newcommand{\bepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\biota}{\boldsymbol{\iota}}
\newcommand{\bXi}{\boldsymbol{\Xi}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}

\newcommand{\qtilde}{\smash{\tilde{q}}}
\newcommand{\ptilde}{\smash{\tilde{p}}}

\newcommand{\bxhat}{\hat{\mathbf{x}}}
\newcommand{\bXhat}{\hat{\mathbf{X}}}
\newcommand{\byhat}{\hat{\mathbf{y}}}
\newcommand{\bYhat}{\hat{\mathbf{Y}}}

\newcommand{\bxbar}{\bar{\mathbf{x}}}
\newcommand{\bXbar}{\bar{\mathbf{X}}}
\newcommand{\bybar}{\bar{\mathbf{y}}}
\newcommand{\bYbar}{\bar{\mathbf{Y}}}






\newcommand{\pms}[1]{\ensuremath{{\scriptstyle\pm #1}}}


\usepackage{standalone}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgf}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
\usetikzlibrary{angles,quotes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{fit}
\usetikzlibrary{arrows}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{shapes.symbols}
\usetikzlibrary{shadings}
\usetikzlibrary{shapes}
\usetikzlibrary{fadings}
\usetikzlibrary{bayesnet}
\usetikzlibrary{matrix}
\usetikzlibrary{plotmarks}
\usetikzlibrary{intersections}
\usetikzlibrary{pgfplots.fillbetween}
\pgfplotsset{compat=1.14}
%
\usepackage{siunitx}

\usepackage{colortbl}
\definecolor{mediumgray}{gray}{0.7}
\definecolor{lightgray}{gray}{0.85}
\definecolor{lightlightgray}{gray}{0.9}
\definecolor{C1}{HTML}{1F77B4}
\definecolor{C2}{HTML}{FF7F0E}
\definecolor{C3}{HTML}{2CA02C}
\definecolor{C4}{HTML}{D62728}
\definecolor{C5}{HTML}{9467BD}
\colorlet{C1light}{C1!70!white}
\colorlet{C2light}{C2!70!white}
\colorlet{C3light}{C3!70!white}
\colorlet{C4light}{C4!70!white}
\colorlet{C5light}{C5!70!white}
\colorlet{C1lighter}{C1!50!white}
\colorlet{C2lighter}{C2!50!white}
\colorlet{C3lighter}{C3!50!white}
\colorlet{C4lighter}{C4!50!white}
\colorlet{C5lighter}{C5!50!white}
\colorlet{C1vlight}{C1!20!white}
\colorlet{C2vlight}{C2!20!white}
\colorlet{C3vlight}{C3!20!white}
\colorlet{C4vlight}{C4!20!white}
\colorlet{C5vlight}{C5!20!white}
\colorlet{linkcolor}{violet}
% \colorlet{citecolor}{RedOrange}  %
% \colorlet{urlcolor}{Aquamarine}

\newtheorem{approximation}{Approximation}

%%%%%%% TEXT ACRONYMS

\newcommand{\dgps}{\textsc{dgp}s\xspace}
\newcommand{\dgp}{\textsc{dgp}\xspace}
\newcommand{\gps}{\textsc{gp}s\xspace}
\newcommand{\gp}{\textsc{gp}\xspace}
\newcommand{\bnn}{\textsc{bnn}\xspace}
\newcommand{\bnns}{\textsc{bnn}s\xspace}
\newcommand{\np}{\textsc{np}\xspace}
\newcommand{\nps}{\textsc{np}s\xspace}
\newcommand{\vae}{\textsc{vae}\xspace}
\newcommand{\vaes}{\textsc{vae}s\xspace}
\newcommand{\iwvae}{\textsc{iwvae}\xspace}
\newcommand{\iwvaes}{\textsc{iwvae}s\xspace}
\newcommand{\vi}{\textsc{vi}\xspace}
\newcommand{\svi}{\textsc{svi}\xspace}
\newcommand{\dsvi}{\textsc{dsvi}\xspace}
\newcommand{\fsvi}{\textsc{fsvi}\xspace}
\newcommand{\psvi}{\textsc{psvi}\xspace}
\newcommand{\iwvi}{\textsc{iwvi}\xspace}
\newcommand{\snr}{\textsc{snr}\xspace}
\newcommand{\snrs}{\textsc{snr}s\xspace}
\newcommand{\dreg}{\textsc{dreg}\xspace}
\newcommand{\clt}{\textsc{clt}\xspace}
\newcommand{\elbo}{\textsc{elbo}\xspace}
\newcommand{\elbos}{\textsc{elbo}s\xspace}
\newcommand{\kld}{KL divergence\xspace}
\newcommand{\fsgc}{\textsc{fsgc}\xspace}
\newcommand{\psmap}{\textsc{ps-map}\xspace}
\newcommand{\jsd}{JS divergence}



\usepackage{tcolorbox}

\newcommand{\hypothesis}[2]{%
\begin{tcolorbox}[colback=blue!10!white,leftrule=2.5mm,size=title]
\textbf{#1}: #2
\end{tcolorbox}
\vspace{-0.1cm}%
}

==> include/tech_report_watermark.tex <==
% Load the necessary packages
\usepackage{background}
\usepackage{ifthen}

% Define the text to be placed in the top right corner
\backgroundsetup{
  scale=1,
  color=black,
  opacity=1,
  angle=0,
  position=current page.north east,
  hshift=-0.8cm,
  vshift=-0.8cm,
  nodeanchor=north east,
  contents={%
    \ifthenelse{\value{page}=1}{% Check if it's the first page
      \begin{minipage}{.2\paperwidth}
        \raggedleft
        \fontsize{8pt}{10pt}\selectfont % Adjust the font size here (8pt)
        \sffamily % Change the font to sans-serif
        TECHNICAL REPORT\\
        R-0\\
        Apr 2023
      \end{minipage}%
    }{}% If it's not the first page, display nothing
  }
}

